Worst-Case Welfare of Item Pricing in the Tollbooth Problem

We study the worst-case welfare of item pricing in the \emph{tollbooth problem}. The problem was first introduced by Guruswami et al, and is a special case of the combinatorial auction in which (i) each of the $m$ items in the auction is an edge of some underlying graph; and (ii) each of the $n$ buyers is single-minded and only interested in buying all edges of a single path. We consider the competitive ratio between the hindsight optimal welfare and the optimal worst-case welfare among all item-pricing mechanisms, when the order of the arriving buyers is adversarial. We assume that buyers own the \emph{tie-breaking} power, i.e. they can choose whether or not to buy the demand path at 0 utility. We prove a tight competitive ratio of $3/2$ when the underlying graph is a single path (also known as the \emph{highway} problem), whereas item-pricing can achieve the hindsight optimal if the seller is allowed to choose a proper tie-breaking rule to maximize the welfare. Moreover, we prove an $O(1)$ upper bound of competitive ratio when the underlying graph is a tree. For general graphs, we prove an $\Omega(m^{1/8})$ lower bound of the competitive ratio. We show that an $m^{\Omega(1)}$ competitive ratio is unavoidable even if the graph is a grid, or if the capacity of every edge is augmented by a constant factor $c$. The results hold even if the seller has tie-breaking power.

==> general_case.tex <==
\section{General Set Packing}
\label{sec: general case}

In this section we consider the general case. We denote by $U=\set{1,\ldots,n}$ the ground set of items, and for each $1\le j\le m$, we denote by $S_j$ be the demand set of buyer $B_j$, and let $v_j$ be its value. 
%We denote $\sset=\set{S_1,S_2,\ldots,S_m}$.
The main result in this section is summarized in the following theorem.

\begin{theorem}
\label{thm:general_case}
For any given buyer-profile $\fset=\set{(S_j,v_j)}_{1\le j\le m}$, there exists a set of prices on items of $U$, that achieves worst-case revenue at least $\Omega(\opt(U,\fset)/\sqrt{n})$, even without the power of tie breaking.
\end{theorem}

\begin{proof}
Let $\sset=\set{S_1,\ldots,S_m}$. 
We say that a subset $\tilde \sset$ of $\sset$ is \emph{independent} iff the sets in $\tilde\sset$ are mutually disjoint.
Let $\sset^*$ be the independent subset of $\sset$ that, over all independent subsets of $\sset$, maximizes the total value, namely $\sset^*=\arg_{\tilde \sset \subseteq \sset: \tilde \sset \text{ is independent}}\max\set{\sum_{S_j\in \tilde\sset}v_j}$. 
We denote $\sset^*=\set{S_{j_1},\ldots,S_{j_t}}$, $J=\set{j_1,\ldots,j_t}$ and $\hat S=\bigcup_{j\in J}S_J$, so $\opt(U,\fset)=\sum_{j\in J}v_j$.
Let $p=\set{p(i)}_{1\le i\le n}$ be a set of prices. We say that a demand set $S_j$ \emph{survives} the price $p$, or that the buyer $B_j$ can \emph{afford} her demand set $S_j$ under the price $p$, iff $v_j>p(S_j)=\sum_{i\in S_j}p(i)$. For convenience, we sometimes refer to $v_j$ by $v(S_j)$.

For brevity, we denote $\opt=\opt(U,\fset)$. 
We compute the prices that achieves worst-case revenue $\Omega(\opt/\sqrt{n})$ in two steps.
In the first step, for each item that does not belong to set $\hat S$, we set its price to be $+\infty$; while for each item in $\hat S$, we set its price to be $\optwel/100|\hat S|$. Denote by $\sset'$ the set of all demand sets that survive the prices set in the first step.
Clearly, each set in $\sset'$ is a subset of $\hat S$.
We show in the following claim that the sets of $\sset^*$ that survive the prices in the first step contain most of the value in $\sset^*$.
\begin{observation}
\label{obs:most_value_survive}
$\sum_{S\in (\sset^*\cap \sset')}v(S)\ge 0.99\cdot\optwel$.
\end{observation}
\begin{proof}
By definition, 
$$\sum_{S\in \sset^*\setminus \sset'}v(S)\le \sum_{S\in \sset^*\setminus \sset'}p(S)\le 
\frac{\optwel}{100|\hat S|}\cdot \left(\sum_{S\in \sset^*\setminus \sset'}|S|\right)
\le 
\frac{\optwel}{100|\hat S|}\cdot |\hat S|=0.01\cdot \optwel,
$$
where the last inequality is because the subset $\sset^*$ is independent and the sets in $\sset^*$ are all subsets of $\hat S$. It follows that 
$\sum_{S\in (\sset^*\cap \sset')}v(S)=\sum_{S\in \sset^*}v(S)-\sum_{S\in (\sset^*\setminus \sset')}v(S)\ge \opt-0.01\cdot\opt= 0.99\cdot\optwel$.
\end{proof}

In the second step, we first compute a hitting set $H$ of sets in $\sset'$ with minimum size. Specifically, we compute (by brute force) a subset $H$ of $\hat S$ that, among all subsets of $\hat S$ that intersects every set in $\sset'$,  minimizes the cardinality.
We distinguish between two cases, depending on whether or not $|H|$ is sufficiently large.

\textbf{Case 1. $|H|>\sqrt{n}$.}
In this case we simply let the prices set in the first step be the final prices of the items. We claim that these prices guarantee the worst-case revenue of at least $0.01\cdot\optwel/\sqrt{n}$. To see this, notice that (i) for every set $S_j\notin \sset'$, whenever buyer $B_j$ comes, she cannot afford her demand set $S_j$ (since $p(S_j)=+\infty>v(S_j)$); and (ii) no matter in what order come the buyers, the set of sold items in $\hat S$ at the end of the selling process must form a hitting set of all sets of $\sset'$ (since otherwise there exists a set $S_j\in \sset'$ with none of its items sold at the end of the selling process; but then when buyer $B_j$ comes in the selling process, all items of $S_j$ are available, and $p(S_j)<v_j$, a contradiction). Therefore, the number of sold items in $\hat S$ is at least $\sqrt{n}$. Recall that each item in $\hat S$ was priced $\optwel/100|\hat S|$, we can therefore conclude that the revenue is at least 
$\sqrt{n}\cdot(\optwel/100|\hat S|)\ge 0.01\cdot\optwel/\sqrt{n}$.

\textbf{Case 2. $|H|\le \sqrt{n}$.}
In this case, for each item $i\in H$, we increase the current price of $i$ (which is the price of item $i$ set in the first step) by $\optwel/100|H|$. We let these modified prices be the final prices.
We first show in that there exists at least one set in $\sset^*\cap \sset'$ that survives $\tilde p$.
Assume for contradiction that no sets in $\sset^*\cap \sset'$ survived the price $\tilde p$. 
Since the sets in $\sset^*\cap \sset'$ are mutually disjoint, 
$$\sum_{S\in (\sset^*\cap \sset')} v(S)\le 
\sum_{S\in (\sset^*\cap \sset')} \tilde p(S) \le
\frac{\optwel}{100|\hat S|}\cdot |\hat S|+ \frac{\optwel}{100|H|}\cdot|H|\le 0.02\cdot\optwel,$$
a contradiction to Observation~\ref{obs:most_value_survive}.
As a result, at least one set in $\sset'$ survives $\tilde p$, and therefore, at the end of the the selling process, at least one buyer will get her demand set (which is not necessarily a set in $\sset^*\cap \sset'$).
On the other hand, since each set in $\sset'$ contains an item in $H$, the price for each set in $\sset'$ is at least $\optwel/100|H|\ge 0.01\cdot\optwel/\sqrt{n}$.
Therefore, we will obtain revenue at least $0.01\cdot\optwel/\sqrt{n}$.
\end{proof}



We complement Theorem~\ref{thm:general_case} with the following theorem.


\begin{theorem}\label{thm:general_hardness}
For each integer $n>0$, there is a buyer-profile $\fset=\set{(S_j,v_j)}_{1\le j\le m}$, such that any set of prices on items of $U$ can achieve worst-case revenue at most $O(\opt(U,\fset)/\sqrt{n})$, even with the power of tie breaking.
\end{theorem}

\begin{proof}
Let $r$ be the largest integer such that $n\ge \binom{r}{2}$, so $r=\Theta(\sqrt{n})$.
Let $K_r$ be a complete graph on $r$ vertices, and denote its vertex set by $V(K_r)=\set{u_1,u_2,\ldots,u_r}$.
The ground set is defined to be the union of the set of all edges in $K_r$ and some other arbitrary $n-\binom{r}{2}$ elements, namely $E(K_r)\subseteq U$. There are $r+1$ buyers $B_0,B_1,\ldots,B_{r}$. The buyer $B_0$ demands the set of all edges, namely $S_0=E(K_r)$, with value $v_0=1$. For each $1\le i\le r$, the buyer $B_i$ demands the set of incident edges of vertex $u_i$, namely $S_i=\set{(u_i,u_j)\mid 1\le j\le r, j\ne i}$), with value $v_i=3/r$.

Since for any $1\le j_1 < j_2\le r$, the demand sets $S_{j_1}$ and $S_{j_2}$ intersect, the optimal allocation is to assign all edges to buyer $B_0$, so $\opt(U,\fset)=1$. However, as we will show now, any set $\set{p(e)}_{e\in E(K_r)}$ of prices will only guarantee to achieve revenue at most $3/r$.
In fact, if there exists $1\le j\le r$, such that $p(S_j)=\sum_{e\in S_j}p(e)< 3/r$, then we let the buyer $B_j$ comes first, so $B_j$ will get her demand set $S_j$ at price less than $3/r$. Since $S_j$ intersects every other demand set, no matter in what order come the other buyers, the revenue obtained by this selling process is at most $3/r$. Consider now the case where for each $1\le j\le r$, $p(S_j)\ge 3/r$.
Since every edge appears in exactly two demand sets of $\set{S_1,\ldots,S_r}$, $p(S_0)=\sum_{1\le j\le r}p(S_j)/2$, so $p(S_0)\ge r(3/r)/2=3/2>1$ and buyer $B_0$ cannot afford her demand set, either.
Therefore, in this case the selling process ends up achieving revenue $0$.
\end{proof}

==> literature_review.tex <==
\subsection{Motivation: The Walrasian Equilibrium}
\subsubsection{Definition}
$n$ items, $m$ buyers. Each buyer has a fixed valuation $v:2^{[n]}\to \mathbb{R}$.

Price $p\in\mathbb{R}^n$ for each item.

Demand set: $D(v_i,p)=\arg\max_{S\subseteq[n]}(v_i(S)-p(S))$, i.e. the utility-maximizing set.

Market Equilibrium: disjoint $S_1,\cdots,S_m$, $S_i\in D(v_i,p)$, $\cup S_j=[n]$.

First welfare theorem: In equilibrium, the welfare is maximized.

Gross substitutes valuations $v$: for any $p\leq p'$ and $S\in D(v,p)$, there exists $X\in D(v,p')$ such that $S\cap\{i|p_i=p'_i\}\subseteq X$.

Some examples of GS valuation function:
\begin{itemize}
    \item Unit-demand
    \item Additive
    \item Matching valuations: $v(S)=$ maximum matching from $S$
\end{itemize}
GS is a subclass of submodular functions.

\subsection{Existence of Equilibrium}
\begin{theorem}
\ [Kelso-Crawford '82] When all agents have GS valuations, then Walrasian Equilibrium always exists.
\end{theorem}

Walrasian Equilibrium does not exist beyond GS valuation, see the following theorem.
\begin{theorem}
\ [Gul-Stachetti '00](seemingly with error, reproved by [Berger-Eden-Feldman '20]) If $v_1$ is not GS, then there exists unit-demand buyers $v_2,\cdots, v_n$ such that $(v_1,\cdots,v_n)$ does not have Walrasian Equilibrium.
\end{theorem}


\begin{theorem}\label{thm:lp}
\ [Nisan-Segal '06] Walrasian Equilibrium exists iff the LP for welfare maximization has integral optimal solution. \\
$\max\sum_{i,S}v_{i}(S)x_{iS}$ 
\end{theorem}
Theorem~\ref{thm:lp} is the literature that formulates the problem using primal and dual lp, and relates the dual variables to prices and utilities. 

There should be more theorems on the existence of Walrasian equilibrium beyond GS, see ``Why Prices Need Algorithms'' by Roughgarden and Talgam-Cohen.

\subsubsection{Approximation of Walrasian Equilibrium via Prophet Inequality}
\begin{theorem}
\ [Feldman-Gravin-Lucier '15] When all agents have XOS (fractionally subadditive) valuations, then static item pricing gives 2-approx in welfare. Works even for Bayesian setting.
\end{theorem}
\begin{theorem}
\ [Dütting-Kesselheim-Lucier '20] When all agents have subadditive valuations, then static item pricing gives $O(\log\log n)$-approx in welfare. Works even for Bayesian setting.
\end{theorem}
Main open question: When all agents have subadditive valuations, can static item pricing give $O(1)$-approx in welfare, even for fixed valuation?

\subsection{Hardness Results}
\begin{theorem}
\ [Feldman-Gravin-Lucier '15] When all agents demands intervals of size at most $n$, item pricing cannot do better than $n$-approx. (One single minded buyer demanding the entire interval with value $n-\eps$, another unit-demand buyer demanding each item with value 1.)
\end{theorem}
\begin{theorem}
\ [Trevisan '01] Computational hardness result: $o(k/2^{O(\sqrt{\log k})})$-approx integral offline allocation for single-minded buyers that demands sets of size at most $n$ cannot be found efficiently, via reduction to maximum independent set, even in the case where all demand-sets have size at most $k$.
\end{theorem}

==> no_tie_breaking.tex <==
\section{Competitive Ratios without the Tie-Breaking Power}\label{sec:no_tie_breaking}

In this section, we consider the scenario where the seller does not have the tie-breaking power. 
%Due to the space limit, all proofs in this section will be postponed to Appendix~\ref{sec:appx_no_tie_breaking}.




\subsection{Path}\label{sec:pathnt}

We first focus on the case when $G$ is a single path. Unlike the scenario with tie-breaking power, where the optimal welfare can be obtained with some set of prices (Theorem~\ref{thm:path}), the competitive ratio may be strictly larger than 1 when the seller has no tie-breaking power.

\begin{theorem}\label{thm:path_no_tie_hardness}
\label{thm: path_no_tie_lower_bound}
$\rationt(\pathh)\geq 3/2$, i.e. there exists a path graph $G$ and an instance $\fset$, such that any set of prices achieves worst-case welfare at most $2/3\cdot \opt(G,\fset)$, when the seller has no tie-breaking power.
\end{theorem}
\begin{proof}
Let $G$ be a path consisting of three edges $e_1,e_2,e_3$, that appears on the path in this order. The instance is described below.
\begin{itemize}
\item Buyer 1 demands the path consisting of a single edge $e_1$, with value $1$;
\item Buyer 2 demands the path consisting of a single edge $e_3$, with value $1$;
\item Buyer 3 demands the path consisting of edges $e_1,e_2$, with value $2$; and
\item Buyer 4 demands the path consisting of edges $e_2,e_3$, with value $2$.
\end{itemize}
	
It is clear that the optimal allocation is assigning $e_1$ to buyer 1 and $e_2,e_3$ to buyer 4 (or assigning $e_3$ to buyer 2 and $e_1,e_2$ to buyer 3). The optimal welfare $\opt(G,\fset)=3$.
We now show that, for any prices $p_1,p_2,p_3$, there is an order $\sigma$ of the four buyers such that the obtained welfare is at most $2$, when the seller has no tie-breaking power. We distinguish between two cases.

\textbf{Case 1. $p_1\leq 1$ and $p_3\leq 1$.} We let buyers 1 and 3 come first and take edges $e_1$ and $e_3$ respectively. Note that the seller does not have the tie-breaking power. The buyer can decide whether or not to take the path when the price equals the value. Now buyers 3 and 4 cannot get their paths. So the obtained welfare is $2$.

\textbf{Case 2. $p_1>1$ or $p_3>1$.} Assume without loss of generality that $p_1>1$. If $p_2+p_3\leq 2$, then we let buyer 4 come first and take edges $e_2$ and $e_3$. It is clear that no other buyer can get her path. So the total welfare is 2. If $p_2+p_3>2$, then $p_1+p_2+p_3>3$. Note that it is impossible in this case all edges are sold, since the hindsight optimal welfare is 3. Therefore, the obtained welfare is at most $2$.
\end{proof}

In Theorem~\ref{thm:path_no_tie} we prove that the competitive ratio $3/2$ is tight for path graphs, when the seller has no tie-breaking power.

\begin{theorem}
\label{thm:path_no_tie}
$\rationt(\pathh)\leq 3/2$. Moreover, the prices that achieve the competitive ratio 3/2 can be computed efficiently.
\end{theorem}
\begin{proof}
From \Cref{thm:path}, (LP-Primal) has an integral optimal solution.  We denote by $y^*$ the integral optimal solution of (LP-Primal)  that maximizes $\sum_{j\in [n]}y^*_j$. Note that $y^*$ can be computed by solving a slightly different LP that is obtained from (LP-Primal) by changing its objective to $\sum_{j\in [n]}(v_j+\eps')\cdot y_j$, for some small enough $\eps'>0$.
Define $Y=\set{j\mid y^*_j=1}$ and
$\qset_Y=\set{Q_j\mid y^*_j=1}$. 

% Let $\eps=\frac{1}{m^2}\cdot\min_jv_j$.
% We prove the following lemma.
% \begin{lemma}\label{lem:price-strictly-positive}
% There is an optimal solution $\set{p^*(e)}_{e\in E(G)}$ for (LP-Dual), such that 
% (i) for each edge $e\in E(\qset_Y)$, $p^*(e)\geq \eps$; and (ii) 
% for each $j\in [n]$, $p^*(Q_j)\geq v_j$.
% \end{lemma}
% \begin{proof}
% We construct another instance $\fset'$ from $\fset$ as follows. We add, for each $e\in E(G)$ a new buyer demanding the path consisting of a single edge $e$ with value $\eps$.
% On one hand, it is easy to see that $y^*$ is still an optimal solution for this new instance. Let $p^*$ be any optimal solution for the corresponding dual LP for the new instance. Clearly, $p^*$ is also an optimal solution of (LP-Dual) and satisfies both properties. 
% \end{proof}

\begin{lemma}\label{lem:price-strictly-positive}
There is an $\eps>0$ and an optimal solution $\set{p^*(e)}_{e\in E(G)}$ for (LP-Dual), such that
(i) for each edge $e\in E(\qset_Y)$, $p^*(e)\geq \eps$; and (ii)
for each $j\in [m]$, either $p^*(Q_j)=v_j$, or $p^*(Q_j)>v_j+m\eps$.
\end{lemma}

\begin{prevproof}{Lemma}{lem:price-strictly-positive}
%Note that picking any optimal solution in (LP-Dual) can only guarantee non-negative prices.
Let $\eps'=\frac{1}{m^2}\cdot\min_jv_j$. We construct another instance $\fset'$ from $\fset$ as follows. We add, for each $e\in E(G)$ a new buyer demanding the path consisting of a single edge $e$ with value $\eps'$.
On one hand, it is easy to see that $y^*$ is still an optimal solution of this new instance. Let $p^*$ be any optimal solution for the corresponding dual LP for the new instance $\fset$. Define $\eps''=\frac{1}{2m}\min_{j:p*(Q_j)>v_j}(p^*(Q_j)-v_j)$ and $\eps=\min\{\eps',\eps''\}$. Clearly $p^*$ is also an optimal dual solution for the instance $\fset$ and satisfies both properties.
\end{prevproof}

Now choose $\eps>0$ and the prices $p^*$ from Lemma~\ref{lem:price-strictly-positive}. We define $A=\set{j\mid v_j=p^*(Q_j)}$ and $\qset_A=\set{Q_j\mid j\in A}$.
\begin{definition}
We say that a set $\qset\subseteq \qset_A$ of edge-disjoint paths is \emph{good}, iff set $\qset_A\setminus \qset$ does not contain another subset $\qset'$ of $|\qset'|\ge 2$ edge-disjoint paths, such that
$\bigcup_{j:Q_j\in \qset'}Q_j=\bigcup_{j:Q_j\in \qset}Q_j$. 
\end{definition}
\mingfeinote{Mingfei: Change the word ``good".}

We prove the following lemma about good edge-disjoint paths.




\begin{lemma}\label{claim:covering_implies_optimal}
There is an efficient algorithm that, given a good set $\qset$ of edge-disjoint paths, computes a set of positive prices $p=\{p(e)\}_{e\in E(\qset)}$
that achieves worst-case welfare at least $\sum_{Q_j\in \qset}v_j$.
\end{lemma}
\begin{proof}
We denote $I=\bigcup_{Q_j\in \qset}Q_j$ and $\qset_I=\{Q_j\in \qset_A\mid Q_j\subseteq I\}$. 
First, for each edge $e\notin E(I)$, we set its price $p(e)=+\infty$. 
Therefore, all buyers $j$ with $Q_j\notin \qset_I$ cannot get her demand path.
We will show that we can efficiently compute prices $\set{p(e)}_{e\in E(I)}$ for edges of $I$, such that (i) for each path $Q_j\in \qset$, $v_j>p(Q_j)$; and (ii) for each path $Q_j\in \qset_I\setminus \qset$, $v_j<p(Q_j)$. 
It is clear that the set $\set{p(e)}_{e\in E(G)}$ of prices achieves worst-case welfare $\sum_{Q_j\in \qset}v_j$.

The existence of prices $\set{p(e)}_{e\in E(I)}$ is equivalent to the feasibility of the following system.
\begin{equation}\label{lp:covering-primal}
\left\{
\begin{array}{cccc}
\displaystyle \sum_{e\in Q_j}p(e) &< & v_j,&\forall Q_j\in\qset;\\
\displaystyle \sum_{e\in Q_j}p(e) & >& v_j,&\forall Q_j\in \qset_I\setminus \qset.
\end{array}
\right.
\end{equation}
From the definition of $A$, and since $\qset_I\subseteq\qset_A$, for each path $Q_j\in \qset_I$, $\sum_{e\in Q_j}p^*(e)= v_j$. 
We denote $\alpha(e)=p(e)-p^*(e)$ for all $e\in E(I)$, then system~\eqref{lp:covering-primal} is feasible if the following system is feasible, for some small enough $\eps'>0$.
\begin{equation}\label{lp:covering-primal2}
\left\{
\begin{array}{cccc}
\displaystyle \sum_{e\in Q_j}\alpha(e) &\le & -\eps',&\forall Q_j\in\qset;\\
\displaystyle \sum_{e\in Q_j}\alpha(e) & \ge & \eps',&\forall Q_j\in \qset_I\setminus \qset.
\end{array}
\right.
\end{equation}
\iffalse
Then system~\eqref{lp:covering-primal2} is feasible if and only if the following system is feasible, for a small enough constant $\sigma>0$.
\begin{equation}\label{lp:covering-primal3}
\left\{
\begin{array}{cccc}
\displaystyle \sum_{e\in Q_j}\alpha(e) &\le & -\sigma,&\forall Q_j\in\qset;\\
\displaystyle \sum_{e\in Q_j}-\alpha(e) & \leq & -\sigma,&\forall Q_j\in \qset_I\setminus \qset.
\end{array}
\right.
\end{equation}
\fi
From Farkas' Lemma,
system~\eqref{lp:covering-primal2} is feasible if and only if the following system is infeasible.
\begin{equation}\label{lp:covering-dual}
\left\{
\begin{array}{rccc}
\displaystyle \sum_{Q_j\in \qset}\beta_j\cdot\mathbbm{1}[e\in Q_j]-\sum_{Q_j\in \qset_I\setminus \qset}\beta_j\cdot\mathbbm{1}[e\in Q_j] &=& 0,&\forall e\in E(I);\\
\displaystyle\sum_{Q_j\in \qset_I}\beta_j&>& 0;\\
\beta_j & \in & [0,1],&\forall Q_j\in \qset_I.
\end{array}
\right.
\end{equation}
where the additional constraints $\beta_j\le 1, \forall Q_j\in \qset_I$ will not influence the feasibility of the system due to scaling.
Next we will prove that system \eqref{lp:covering-dual} is feasible iff it admits an integral solution.

\begin{definition}
We say that a matrix $A$ is \emph{totally unimodular} iff the determinant of every square submatrix of $A$ belongs to $\{0,-1,+1\}$.
\end{definition}
\begin{lemma}[Folklore]
\label{lem:forklore}
If a matrix $A\in \mathbb{R}^{n\times m}$ is totally unimodular and a vector $b\in\mathbb{R}^n$ is integral, then every extreme point of the polytope $\{x\in \mathbb{R}^m\mid Ax\leq b, x\geq 0\}$ is integral.
\end{lemma}

\begin{lemma}[\cite{schrijver1998theory}] \label{lem:proposition-tu}
A matrix $A\in \mathbb{R}^{n\times m}$ is totally unimodular iff for any subset $R\subseteq [n]$, there exists a partition $R=R_1\cup R_2$, $R_1\cap R_2=\emptyset$, such that for any $j\in [m]$,
$$\sum_{i\in R_1}a_{ij}-\sum_{i\in R_2}a_{ij}\in \{0,-1,+1\}.$$
\end{lemma}

\begin{lemma}\label{lem:covering-integral-solu}
System~\eqref{lp:covering-dual} is feasible if and only if it admits an integral solution.
\end{lemma}
\begin{proof}
We prove that the coefficient matrix $C$ in system \eqref{lp:covering-dual} is totally unimodular.\footnote{The second inequality in system \eqref{lp:covering-dual} is strict inequality. We can modify it to an equivalent inequality $\sum_{j:Q_j\in \qset}\beta_j\geq \eps_0$ for some sufficiently small $\eps_0>0$ and then apply Lemma~\ref{lem:forklore}.} For any set of rows $R=\{i_1,i_2,\cdots,i_k\}$ such that $i_1<i_2<\cdots<i_k$, We define the partition $R_1=\{i_1,i_3,i_5,...\}$ be the set with odd index and $R_2=\{i_2,i_4,i_6,...\}$ be the set with even index. For every column $j$, $Q_j$ is an subpath and thus the ones (or -1s for $Q_j\in \qset_I\setminus \qset$) in the vector $(C_{ij})_{i=1}^m$ are consecutive. Hence the difference between $\sum_{i\in R_1}C_{ij}$ and $\sum_{i\in R_2}C_{ij}$ is at most 1. By Lemma~\ref{lem:proposition-tu}, $C$ is totally unimodular.
\end{proof}


Assume for contradiction that  \eqref{lp:covering-dual} is feasible, let $\beta^*\in \set{0,1}^{\qset_I}$ be an integral solution of \eqref{lp:covering-dual}.
Note that the constraints
$\sum_{j:Q_j\in \qset}\beta^*_j\cdot\mathbbm{1}[e\in Q_j]-\sum_{j:Q_j\in \qset_I\setminus \qset}\beta^*_j\cdot\mathbbm{1}[e\in Q_j] = 0,\forall e\in E(I)$ and the fact that paths of $\qset$ are edge-disjoint
imply that the paths in set $\qset'=\{Q_j\mid \beta_j=1\}$ are edge-disjoint. Note that $\qset'\cap\qset=\emptyset$ and $\bigcup_{Q_j\in \qset'}Q_j=\bigcup_{Q_j\in \qset}Q_j$, and this is a contradiction to the assumption that the set $\qset$ is good.
Therefore, system \eqref{lp:covering-dual} is infeasible, and thus system \eqref{lp:covering-primal2} is feasible.
Let $(\alpha(e))_{e\in E(I)}$ be a solution of system~\eqref{lp:covering-primal2}, such that $\sum_{e\in E(I)} |\alpha(e)|\le \eps$. It is clear that such a solution exists due to scaling.
We set $p(e)=p^*(e)+\alpha(e)$ for all $e\in E(I)$, and it is clear that the prices $\set{p(e)}_{e\in E(G)}$ satisfy all the properties of \Cref{claim:covering_implies_optimal}.
Moreover, prices $\set{p(e)}_{e\in E(G)}$ are positive.
\end{proof}

We now complete the proof of Theorem~\ref{thm:path_no_tie} using \Cref{claim:covering_implies_optimal}. 


We denote $\qset_Y=\set{Q_1,Q_2,\ldots,Q_k}$, where the paths are indexed according to the order in which they appear on $G$.
First, for each edge $e\notin E(\qset_Y)$, we set its price $\tilde p(e)=+\infty$.
Therefore, any buyer $j$ with $e\in Q_j$ cannot take her demand path.
In fact, we may assume without loss of generality that $\bigcup_{1\le j\le k}Q_j=G$, since otherwise we can view each connected component (which is also a path) of graph $\bigcup_{1\le j\le k}Q_j$ as the whole graph, and compute prices for its edges separately.

We will compute three sets $\hat\qset_1,\hat\qset_2,\hat\qset_3\subseteq \qset_A$ of edge-disjoint paths, such that 
\begin{enumerate}
\item every edge of $E(G)$ is contained in exactly two paths of $\hat\qset_1,\hat\qset_2,\hat\qset_3$; and
\item \label{prop: good_cover} for each $t\in \set{1,2,3}$, if we further partition the set $\hat\qset_t$ into subsets $\hat\qset^1_t,\ldots,\hat\qset^{r_t}_t$, such the union of the paths in each set $\hat\qset^1_t$ forms a connected component (which is also a path) of graph $\bigcup_{Q_j\in \hat\qset_t}Q_j$, then each of the sets $\hat\qset^1_t,\ldots,\hat\qset^{r_t}_t$ is a good set of edge-disjoint paths. 
\end{enumerate}
By definition, $\sum_{Q_j\in \hat\qset_1}v_j+\sum_{Q_j\in \hat\qset_2}v_j+\sum_{Q_j\in \hat\qset_3}v_j=2\cdot\opt(G,\fset)$.
Assume without loss of generality that $\sum_{Q_j\in \hat\qset_1}v_j\ge (2/3)\cdot\opt(G,\fset)$.
Then from Lemma~\ref{claim:covering_implies_optimal}, there exist prices $\set{\tilde p(e)}_{e\in E(\qset_Y)}$ that achieves worst-case welfare at least $\sum_{Q_j\in \hat\qset_1}v_j\ge (2/3)\cdot\opt(G,\fset)$.

\paragraph{Compute the sets $\hat\qset_1,\hat\qset_2,\hat\qset_3$.}
We now compute the desired sets $\hat\qset_1,\hat\qset_2,\hat\qset_3$ of edge-disjoint paths, which, from the above discussion, completes the proof of Theorem~\ref{thm:path_no_tie}.


We start by defining $\hat\qset$ to be the multi-set that contains, for each path $Q_j\in\qset_Y$, two copies $Q'_j,Q''_j$ of $Q_j$. 
We initially set
\begin{itemize}
\item $\hat\qset_1=\set{Q'_{6r+3},Q'_{6r+4}\mid 1\le r\le k/6} \cup\set{Q''_{6r},Q''_{6r+1}\mid 1\le r\le k/6}$;
\item $\hat\qset_2=\set{Q'_{6r+1},Q'_{6r+2}\mid 1\le r\le k/6} \cup\set{Q''_{6r+4},Q''_{6r+5}\mid 1\le r\le k/6}$; and
\item $\hat\qset_3=\set{Q'_{6r+2},Q'_{6r+3}\mid 1\le r\le k/6} \cup\set{Q''_{6r+2},Q''_{6r+3}\mid 1\le r\le k/6}$.
\end{itemize}
See Figure~\ref{fig:path-1} for an illustration.
Clearly, sets $\hat\qset_1,\hat\qset_2,\hat\qset_3$ partition $\hat\qset$, each contains edge-disjoint paths, and every edge appears twice in paths of $\hat\qset_1,\hat\qset_2,\hat\qset_3$.
However, sets $\hat\qset_1,\hat\qset_2,\hat\qset_3$ may not satisfy Property~\ref{prop: good_cover}.
We will then iteratively modify sets $\hat\qset_1,\hat\qset_2,\hat\qset_3$, such that at the end Property~\ref{prop: good_cover} is satisfied.

Throughout, we also maintain graphs $G_t=\bigcup_{Q\in \hat{\qset}_t}Q$, for each $t\in \set{1,2,3}$. As sets $\hat\qset_1,\hat\qset_2,\hat\qset_3$ change, graphs $G_1,G_2,G_3$ evolve.
We start by scanning the path $G$ from left to right, and process, for each each connected component of graphs $G_1,G_2,G_3$, as follows.

We first process the connected component in $G_1$ formed by the single path $Q_1''$. Clearly, set $\set{Q_1''}$ is good, since if there are other paths $\hat Q,\hat Q'\in \qset_A$ such that $\hat Q,\hat Q'$ are edge-disjoint and $\hat Q\cup \hat Q'=Q_1$, then the set $\set{\hat Q,\hat Q',Q_2,\ldots,Q_k}$ corresponds to another integral optimal solution $\hat y^*$ of (LP-Primal) with $\sum_{j\in [n]}\hat y^*_j=k+1>k=\sum_{j\in [n]}\hat y^*_j$, a contradiction to the definition of $y^*$. We do not modify path $Q''_1$ in $\hat{\qset}_1$ and continue to the next iteration.

We then process the connected component in $G_2$ formed by the paths $Q_1',Q_2'$. If the set $\set{Q_1',Q_2'}$ is good, then we do not modify this component and continue to the next iteration. Assume now that the set $\set{Q_1',Q_2'}$ is not good.
From similar arguments, there exist two other paths $Q^*_1,Q^*_2\in \qset_A$, such that $Q^*_1,Q^*_2$ are edge-disjoint and $Q^*_1\cup Q^*_2=Q_1\cup Q_2$. 
We then replace the paths $Q'_1,Q'_2$ in $\hat{\qset}_2$ by paths $Q^*_1,Q^*_2$.
Let $v^*_1$ be the vertex shared by paths $Q^*_1,Q^*_2$, so $v^*_1\ne v_1$. We distinguish between the following cases.

\textbf{Case 1. $v^*_1$ is to the left of $v_1$ on path $G$.}
As shown in Figure~\ref{fig:path-2}, we keep the path $Q^*_2$ in $\hat{\qset}_2$, and move path $Q^*_1$ to $\hat{\qset}_3$.
Clearly, we create two new connected components: one in $G_3$ formed by a single path $Q^*_1$, and the other in $G_2$ formed by a single path $Q^*_2$.
From similar arguments, the corresponding singleton sets $\set{Q^*_1}, \set{Q^*_2}$ are good.

\textbf{Case 2. $v^*_1$ is to the right of $v_1$ on path $G$.}
As shown in Figure~\ref{fig:path-4}, we keep the path $Q^*_2$ in $\hat{\qset}_2$, move path $Q^*_1$ to $\hat{\qset}_1$ and additionally move the path $Q'_1$ processed in previous iteration to $\hat{\qset}_2$.
Clearly, we create two new connected components: one in $G_1$ formed by a single path $Q^*_1$, and the other in $G_2$ formed by a single path $Q^*_2$.
From similar arguments, the corresponding singleton sets $\set{Q^*_1}, \set{Q^*_2}$ are good. 
Note that we have additionally moved $Q'_1$ to $\hat{\qset}_2$, but since we did not change the corresponding component, the singleton set $\set{Q'_1}$ is still good.

\begin{figure}[h]
\centering
\subfigure[An illustration of paths in set $\hat{\qset}_1\cup \hat{\qset}_2\cup \hat{\qset}_3$ at the beginning.]{\scalebox{0.4}{\includegraphics{interval_1.jpg}}\label{fig:path-1}}
\subfigure[An illustration of path modification in Case 1.]{\scalebox{0.4}{\includegraphics{interval_2.jpg}}\label{fig:path-2}}
\subfigure[An illustration of path modification in Case 2.]{\scalebox{0.4}{\includegraphics{interval_4.jpg}}\label{fig:path-4}}
\subfigure[How old and new paths/components may possibly interact.]{\scalebox{0.39}{\includegraphics{interval_3.jpg}}\label{fig:path-3}}
\caption{Illustrations of the algorithm for computing path sets $\hat{\qset}_1,\hat{\qset}_2,\hat{\qset}_3$.}
\end{figure}

We continue processing the remaining connected components in the same way until all components are good. We will show that, every time a connected component is not good and the corresponding two paths are replaced with two new paths, the connected components in $G_1,G_2,G_3$ that we have processed in previous iterations will stay good. Therefore, the algorithm will end up producing good components in $G_1,G_2,G_3$ consisting of a good set of one or two edge-disjoint paths.

To see why this is true, consider an iteration where we are processing a component consisting of paths $Q''_i, Q''_{i+1}$, and there exists edge-disjoint paths $Q^*_i,Q^*_{i+1}$ such that $Q^*_i\cup Q^*_{i+1}=Q''_i\cup Q''_{i+1}$, while the endpoint $v^*_i$ shared by $Q^*_i$ and $Q^*_{i+1}$ is an endpoint of a processed component, as shown in Figure~\ref{fig:path-3}. 
Note that this is the only possibility that the new components may influence the previous components,
However, we will show that this is impossible. 
Note that $Q''_{i}\in \qset_Y$. 
We denote by $Q^r$ the path with endpoints $v^*_i$ and $v_i$, then clearly paths $Q^*_i, Q^r$ are not in $\qset_Y$, edge-disjoint and satisfy that $Q_{i}=Q^*_i\cup Q^r$.
Consider now the set $(\qset_Y\setminus \set{Q_{i}})\cup \set{Q^*_i, Q^r}$. It is clear that this set corresponds to another integral optimal solution $\hat y^*$ of (LP-Primal) with $\sum_{j\in [n]}\hat y^*_j=k+1>k=\sum_{j\in [n]}\hat y^*_j$, a contradiction to the definition of $y^*$.
\end{proof}




\subsection{Other Special Families of Graphs}\label{sec:specialgraphsnt}

We bound the competitive ratio for the no tie-breaking case, when $G$ is in special families of graphs discussed in Section~\ref{sec:special_graph}. For star and spider graphs, we prove that the competitive ratios are at most $2$ and $7/2$ respectively. 

\begin{theorem}
\label{thm:star}
For any $\eps>0$, $\rationt(\starr)\leq 2+\eps$. Moreover, the prices that achieve the competitive ratio $2+\eps$ can be computed efficiently.
\end{theorem}

\begin{proof}
The optimal allocation can be computed efficiently by ~\cite{tarjan1985decomposition}. Let $\qset$ be the set of paths in the optimal allocation, so $\optwel=\sum_{j:Q_j\in \qset}v_j$.
We set the prices on the edges of $G$ as follows. Let $\eps'=\eps/5$.
For each path $Q_j\in \qset$, if it contains a single edge $e_i$, then we set the price of $e_i$ to be $(1-\eps')\cdot v_j$; if it contains two edges $e_i,e_{i'}$, then we set the price of both $e_i$ and $e_{i'}$ to be $(\frac{1}{2}-\eps')\cdot v_j$.
For each edges that does not belong to any path of $\qset$, we set its price to be $+\infty$.
	
We now show that the above prices will achieve worst-case welfare at least $(\frac{1}{2}-\eps')\cdot\optwel$. For a path $Q_j$ that contains a single edges $e_i$, clearly $e_i$ will be taken by some buyer (not necessarily $j$) at price $(1-\eps')\cdot v_j$, for any arriving order $\sigma$. For a path $Q_{j'}$ that contains two edges $e_{i},e_{i'}$, we notice that buyer $j'$ can afford her demand path. Thus for any order $\sigma$, at least one of $e_{i},e_{i'}$ will be sold at price $(\frac{1}{2}-\eps')\cdot v_{j'}$, otherwise buyer $j'$ must have purchased $Q_{j'}$. Hence for any order $\sigma$, the total price of the sold edges is at least $(\frac{1}{2}-\eps')\cdot\optwel$. Since all buyers have non-negative utility, the worst-case welfare is also at least $(\frac{1}{2}-\eps')\cdot\optwel\geq \frac{\optwel}{2+\eps}$.
\end{proof}


\begin{theorem}\label{thm:spider-no-tiebreak}
For any $\eps>0$, $\rationt(\spider)\leq 7/2+\eps$. Moreover, the prices that achieve the competitive ratio $7/2+\eps$ can be computed efficiently.
\end{theorem}

\begin{proof}
Let $\qset$ be the set of paths in the optimal allocation. 
We define $\qset_1$ to be the set of all paths in $\qset$ that contains the center of the spider, and we define $\qset_2=\qset\setminus \qset_1$. For each path $Q\in \qset_1$, let $j_Q$ be the buyer who is allocated her demand path $Q$ in the optimal allocation. Define $G_Q$ to be the graph obtained by taking the union of all (one or two) legs whose edge sets intersect with $E(Q)$, and we denote $E_Q=E(G_Q)$. Since paths in $\qset_1$ are edge-disjoint, clearly for any $Q,Q'\in \qset_1$, $E_Q\cap E_{Q'}=\emptyset$. For any edge set $E$, let $\fset|_E\subseteq \fset$ be the sub-instance that contains all buyer $j$ where $Q_j$ has edges only in $E$. Then $\opt(G,\fset)=\sum_{Q\in\qset_1}\opt(G_Q,\fset|_{E_Q})$.

Let $e_{Q,1}$ and $e_{Q,2}$ be the two edges that are in Q and has the spider center as one endpoint.\footnote{$e_{Q,1}=e_{Q,2}$ if the spider center is one endpoint of path $Q$.}
Define $G'_Q$ to be the graph with edge set $E'_Q=\{e|e\in E_Q\setminus Q\}$. In other words, $G'_Q$ contains all edges not in $Q$ but in $E_Q$. Clearly we have $\opt(G_Q,\fset|_{E_Q})=\opt(G'_Q,\fset|_{E'_Q})+v_{j_Q}$. Define $G''_Q$ to be the graph with edge set $E''_Q=Q\setminus\{e_{Q,1},e_{Q,2}\}$; in other words, $G''_Q$ is the graph formed edges in $Q$, but excluding the center of the spider. Note that $E_Q=E'_Q\cup E''_Q\cup \{e_{Q,1},e_{Q,2}\}$. See \Cref{fig:spider_proof} for an illustration.

\begin{figure}[h]
	\centering
	\includegraphics[scale=0.12]{spider_proof.jpg}
	\caption{An illustration of edge sets. Edges of $E'_Q$ are shown in green, and edges of $E''_Q$ are shown in red.\label{fig:spider_proof}}
\end{figure}
Let $\alpha_Q=\frac{\opt(G''_Q,\fset|_{E''_Q})}{v_{j_Q}}$. Clearly $\alpha_Q\leq 1$, since $E''_Q\subseteq Q$. We will construct the price vector $p$ as follows. For every $Q\in \qset_1$, we will first construct two price vectors $p_1$ and $p_2$ on $E_Q$. Then depending on the instance, we will either choose $p(e)=p_1(e),\forall e\in E_Q$, or $p(e)=p_2(e),\forall e\in E_Q$. For every $e\not\in \cup_{Q\in \qset_1}E_Q$, we set $p(e)=+\infty$. Now fix any $Q\in \qset_1$ and any $\eps'>0$.  

\paragraph{Construction of $p_1$.} For each $e\in E'_Q$, let $p_1(e)=+\infty$. For each $e\in E''_Q$, let $p_1(e)=p^*(e)+\frac{1}{m}\eps'$, where $p^*=\{p^*(e)\}_{e\in E''_Q}$ is the set of prices from Theorem~\ref{thm:path} on $G''_Q$, whose worst-case welfare is $\opt(G''_Q,\fset|_{E''_Q})$. For $e=e_{Q,1}$ or $e_{Q,2}$, $p_1(e)=\frac{(1-\alpha_Q)v_{j_Q}}{2}-\eps'$. Then no buyer $j$ where $Q_j$ contains an edge in $E'_Q$ can afford her path. Also, we notice that since $p^*$ is the optimal solution in (LP-Dual) for instance $(G''_Q,\fset|_{E''_Q})$, every buyer $j$ where $Q_j$ has edges only in $E''_Q$ satisfies $v_j\leq p^*(Q_j)$. Thus none of them can afford her path in $p_1$, as $p_1(e)<p^*(e)$ for all $e\in E''_Q$.
	Moreover, the total price of edges in $Q$ is $\sum_{e\in E''_Q}p_1(e)+p_1(e_{Q,1})+p_1(e_{Q,2})<\opt(G''_Q,\fset|_{E''_Q})+\eps'+(1-\alpha_Q)v_{j_Q}-2\eps'<v_{j_Q}$.
	Consider any item pricing $p$ such that $p(e)=p_1(e),\forall e\in E_Q$. From the arguments above, only buyer $j$ whose $Q_j$ contains $e_{Q,1}$ or $e_{Q,2}$ may afford her path. Thus at least one of $e_{Q,1}$ and $e_{Q,2}$ must be sold under $p$ at price $\frac{(1-\alpha_Q)v_{j_Q}}{2}-\eps'$, for any buyers' arriving order $\sigma$. Otherwise, all edges in $E''_Q$ must also be unsold and buyer $j_Q$ should have purchased her path $Q$, contradiction. Thus the contributed welfare from edges in $E_Q$ is at least $\frac{(1-\alpha_Q)v_{j_Q}}{2}-\eps'$.

\paragraph{Construction of $p_2$.} For each $e\in E'_Q\cup E''_Q$, let $p_2(e)$ be the price of edge $e$ by applying Theorem~\ref{thm:path_no_tie} to $G'_Q\cup G''_Q$, which is a union of at most two path graphs. For $e=e_{Q,1}$ or $e_{Q,2}$, set $p_2(e)=+\infty$.
Then by Theorem~\ref{thm:path_no_tie},
if $p(e)=p_2(e),\forall e\in E_Q$,
the contributed welfare from edges in $E_Q$ is at least $\frac{2}{3}\opt(G'_Q\cup G''_Q,\fset|_{G'_Q\cup G''_Q})= \frac{2}{3}\opt(G'_Q,\fset|_{G'_Q})+\frac{2}{3}\opt(G''_Q,\fset|_{G''_Q})=\frac{2}{3}\opt(G'_Q,\fset|_{E'_Q})+\frac{2}{3}\alpha_Qv_{j_Q}$, for any buyers' arriving order $\sigma$. 

Now for any $Q\in \qset_1$, we choose the price with a higher contributed welfare: If $\frac{(1-\alpha_Q)v_{j_Q}}{2}-\eps'>\frac{2}{3}\opt(G'_Q,\fset)+\frac{2}{3}\alpha_Qv_{j_Q}$, we choose $p(e)=p_1(e),\forall e\in E_Q$ and choose $p(e)=p_2(e)$ otherwise. Thus the worst-case welfare of item pricing $p$ is at least
\begin{eqnarray*}
& &\sum_{Q\in \qset_1}\max\left(\frac{(1-\alpha)v_{j_Q}}{2}-\eps',\frac{2}{3}\opt(G'_Q,\fset|_{E'_Q})+\frac{2}{3}\alpha_Qv_{j_Q}\right)\\
&\geq&\sum_{Q\in \qset_1}\frac{4}{7}\left(\frac{(1-\alpha)v_{j_Q}}{2}-\eps'\right)+\frac{3}{7}\left(\frac{2}{3}\opt(G'_Q,\fset|_{E'_Q})+\frac{2}{3}\alpha_Qv_{j_Q}\right)\\
&=&\sum_{Q\in \qset_1}\left(\frac{2}{7}v_{j_Q}+\frac{2}{7}\opt(G'_Q,\fset|_{E'_Q})-\frac{4}{7}\eps'\right)\\
&=&\sum_{Q\in \qset_1}\left(\frac{2}{7}\opt(G_Q,\fset|_{E_Q})-\frac{4}{7}\eps'\right)>\frac{2}{7}\opt(G,\fset)-\frac{4m}{7}\eps'.
\end{eqnarray*}
Choosing $\eps'=\frac{\eps\cdot \opt(G,\fset)}{10m}$ finishes the proof. By~\cite{tarjan1985decomposition}, the optimal allocation for any instance on trees can be computed efficiently. Thus the price vector $p$ can also be computed efficiently according to the construction above.
\end{proof}

For trees, we prove that the competitive ratio is at most 7. Theorem~\ref{thm:tree-no-tiebreak} follows directly from Lemma~\ref{lem:treetospider} and Theorem~\ref{thm:spider-no-tiebreak}.

\begin{theorem}\label{thm:tree-no-tiebreak}
For any $\eps>0$, $\rationt(\tree)\leq 7+\eps$. Moreover, the prices that achieve the competitive ratio $7+\eps$ can be computed efficiently.
\end{theorem}


For cycles, it is easy to prove that $\rationt(\cycle)\leq 3$, if we apply Theorem~\ref{thm:path_no_tie} instead of Theorem~\ref{thm:path} in the proof of Theorem~\ref{thm:cycle}. 
In fact, we show in the following theorem that $\rationt(\cycle)\leq 2$, with a more careful analysis. Thus by Theorem~\ref{thm: cycle_lower_bound}, the competitive ratio 2 is also tight for the no tie-breaking case.

\begin{theorem}
\label{thm:cycle_without_tie}
$\rationt(\cycle)\leq 2$. Moreover, the prices that achieve the competitive ratio $2$ can be computed efficiently.
\end{theorem}

\begin{proof}
Let $\qset^*$ be the subset of $\set{Q_1,\ldots,Q_n}$ that, over all subsets of edge-disjoint paths in $\set{Q_1,\ldots,Q_n}$ that maximizes its total value, maximizes its cardinality. For every $Q\in \qset^*$, let $v(Q)$ be the value of the buyer who receives demand path $Q$ in the optimal allocation $\qset^*$. So $\opt(G,\fset)=\sum_{Q\in \qset^*}v(Q)$.
We distinguish between the following cases.

\textbf{Case 1. $\bigcup_{Q\in \qset^*}Q \ne G$.} Let $e'$ be an edge of $G$ that does not belong to any path of $\qset^*$. We first set the price of $e'$ to be $p(e')=+\infty$. Since $G\setminus e$ is a path, from Theorem~\ref{thm:path_no_tie}, there exist prices $\set{p(e)}_{e\in G\setminus e'}$  that achieves the worst-case welfare $\frac{2}{3}\cdot\sum_{Q\in \qset^*}v(Q)=\frac{2}{3}\cdot \opt(G,\fset)$.

\textbf{Case 2. $\bigcup_{Q\in \qset^*}Q = G$ and $|\qset^*|\ge 4$.} Let $Q'\in \qset^*$ be the path of $\qset^*$ with minimum value.
Since $|\qset^*|\ge 4$, $\sum_{Q\in \qset^*}v(Q)\ge \frac 3 4 \cdot\opt(G,\fset)$. We first set the prices for all edges of $Q'$ to be $+\infty$. We then consider the graph $G\setminus Q'$. From the similar analysis as in Case 1, we get that there exist prices $\set{p(e)}_{e\in G\setminus Q'}$  that achieves the worst-case welfare $\frac{2}{3}\cdot\sum_{Q\in \qset\setminus\set{Q'}}v(Q)=\frac{2}{3}\cdot\frac 3 4\cdot \opt(G,\fset)=\opt(G,\fset)/2$.

\textbf{Case 3. $\bigcup_{Q\in \qset^*}Q = G$ and $|\qset^*|=2$.} Let $Q$ be the path in $\qset^*$ with largest value, so $v(Q)\ge \opt(G,\fset)/2$. We first set the prices for all edges of $G\setminus Q$ to be $+\infty$. From the choice of $\qset^*$, there does not exist a set of edge-disjoint demand paths, whose union is exactly $Q$ and total value equals $v(Q)$. From \Cref{claim:covering_implies_optimal}, there exist prices $\set{p(e)}_{e\in Q}$ that achieves the worst-case welfare $v(Q)\ge \opt(G,\fset)/2$.

\textbf{Case 4. $\bigcup_{Q\in \qset^*}Q = G$ and $|\qset^*|=3$.} Denote $\qset^*=\set{Q_1,Q_2,Q_3}$, where the endpoints for paths $Q_1$ ($Q_2$ and $Q_3$, resp.) are $a,b$ ($b,c$ and $c,a$, resp.).
If some path of $\qset^*$ has value less than $\opt(G,\fset)/4$, then we set the prices for all edges of this path to be $+\infty$, and then from the similar analysis in Case 2, there exist prices $\set{p(e)}_{e\in G\setminus Q'}$  that achieves the worst-case welfare at least $\opt(G,\fset)/2$.
Now assume that $v(Q_1),v(Q_2),v(Q_3)\ge \opt(G,\fset)/4$.
Let $Q'_1=Q_2\cup Q_3$. If there does not exist a set of two edge-disjoint demand paths, whose union is exactly $Q'_1$ and total value equals $v(Q'_1)$, then we set the prices for all edges of $Q_1$ to be $+\infty$, and then from the similar analysis in Case 3, there exist prices $\set{p(e)}_{e\in G\setminus Q'}$  that achieves the worst-case welfare $v(Q_2)+v(Q_3)\ge \opt(G,\fset)/2$.
Therefore, there exist demand paths $P_1,P'_1$ with $P_1\cup P'_1=Q_2\cup Q_3$ and $v(P_1)+v(P'_1)=v(Q_2)+v(Q_3)$.
Similarly, there exist demand paths $P_2,P'_2$ with $P_2\cup P'_2=Q_3\cup Q_1$ and $v(P_2)+v(P'_2)=v(Q_3)+v(Q_1)$; and there exist demand paths $P_3,P'_3$ with $P_3\cup P'_3=Q_1\cup Q_2$ and $v(P_3)+v(P'_3)=v(Q_1)+v(Q_2)$.
Now consider the path $P_1,P'_1,P_2,P'_2,P_3,P'_3$.
For similar reasons, the value of each of these paths is at least $\opt(G,\fset)/4$.
From the above discussion, the union of them contains each edge of $G$ exactly twice. Therefore, either $P_1\cup P'_1\cup P_2$ or $P'_2\cup P_3\cup P'_3$ is a path of $G$ with total value at least $\frac{3}{4}\cdot\opt(G,\fset)$. From similar analysis in Case 2, there exist prices $\set{p(e)}_{e\in G\setminus Q'}$  that achieves the worst-case welfare $\frac{2}{3}\cdot\frac 3 4\cdot \opt(G,\fset)=\opt(G,\fset)/2$.
\end{proof}

At the last of this section, we consider outerplanar graphs. We show that the competitive ratio for any instance in the outerplanar graph is also $O(\log^2 m)$, in the no tie-breaking case. The proof of Theorem~\ref{thm:outerplanar_without_tie} is the same as Theorem~\ref{thm:outerplanar_lower}, with the only difference of applying Theorem~\ref{thm:spider-no-tiebreak} instead of Theorem~\ref{thm:spiderimproved} for spider graphs. The proof is omitted. 

\begin{theorem}
\label{thm:outerplanar_without_tie}
$\rationt(\outerplanar)=O(\log^2 m)$.
\end{theorem}

==> path.tex <==

\subsection{Paths}\label{sec:path}
In this section we consider the case where $G$ is a path. 
Let $E(G)=\set{e_1,\ldots,e_n}$, where the edges are indexed according to the order in which they appear on the path.
%We denote by $\fset=\set{(Q_j,v_j)}_{j\in [m]}$ the buyer-profile.
%It was shown in \cite{chawla2017stability} that, if the seller has the power of tie-breaking, then there exist prices on edges of $G$ that achieves revenue $\opt(G,\fset)$, and such a set of prices can be computed efficiently. 
The following theorem was proved in \cite{chawla2017stability}.
%The first main result in this section is the following theorem, whose proof is provided in \Cref{apd: Proof of thm:path}.
For completeness, we provide its proof in \Cref{apd: Proof of thm:path}.
\begin{theorem}
[Corollary of Lemma 2.1 in \cite{chawla2017stability}]
\label{thm:path}
%If the seller has the power of tie-breaking, then for any
There is an efficient algorithm, that, given any path graph $G$ and any buyer-profile $\fset=\set{(Q_j,v_j)}_{j\in [m]}$, computes a set of prices on edges of $G$ that achieves worst-case welfare $\opt(G,\fset)$, with the power of tie-breaking. Moreover, (LP-Primal) has an integral optimal solution.
\end{theorem}
%In \cite{chawla2017stability}, the authors first proved that (LP-Primal) has an integral optimal solution, and then \Cref{thm:path} directly follows from Lemma~\ref{lem:rounding}. 



\notshow{

\begin{proof}
%Let $e_1,\ldots,e_L$ be the edges of the path $G$, where the edges are indexed according to their appearance in $G$.
%For each $1\le i\le L$, let $x_i$ be the indicator event that the edge $e_i$ is taken by some buyer.
Consider the following linear program.
\begin{eqnarray*}
	\mbox{(P)}	&\text{maximize }
	\sum_{j\in [m]}v_j\cdot y_j\\
	\mbox{s.t.}
	&\sum_{j: e_i\in Q_j}y_j\leq 1&\forall\text{ }1\le i\le L\\
	& y_j\ge 0&\forall\text{ } j\in [m]
\end{eqnarray*}
\begin{claim}\label{thm:lp-primal}
(P) has an integral optimal solution.
\end{claim}
\begin{proof}
%{\color{red} Todo}
The inequalities $\sum_{j: e_i\in Q_j}y_j\leq 1$ are equivalent to $A\textbf{y}\leq \textbf{1}$, where matrix $A=(A_{ij})_{i,j}$ satisfies $A_{ij}=\indicator[x_i\in Q_j], \forall i\in [L],j\in [m]$. Note that $A$ is a 0-1 matrix, where 1s appear consecutively in every row. Thus $A$ is totally \todo{Todo} unimodular. Every vertex in the feasible polytope is an integral solution. Thus (LP-Primal) has an integral optimal solution.
\end{proof}
%Below is the Dual LP for (LP-Primal).
The dual of (LP-Primal) is as follows:
\begin{eqnarray*}
	\mbox{(LP-Dual)}	&\text{minimize }
	\sum_{1\le i\le L}p_i\\
	\mbox{s.t.}
	&\sum_{i: e_i\in Q_j}p_i\geq v_j&\forall\text{ } j\in [m]\\
	& p_i\ge 0&\forall\text{ } 1\le i\le L
\end{eqnarray*}
Let $y^*$ be any optimal integral solution for (LP-Primal), and
let $p^*=\{p_i^*\}_{i\in [L]}$ be any optimal solution for (LP-Dual). Then by strong duality, $\sum_{j}v_jy^*_j=\sum_{i}p^*_i=\optwel$.
Moreover, from the complementary slackness, for each $j\in [m]$ such that $\sum_{i: e_i\in Q_j}p^*_i>v_j$, we have $y^*_j=0$.
%We solve the above two linear programs and obtain an integral optimal solution $y^*$ for (LP-Primal) and an optimal solution $p^*$ for (LP-Dual).
%We then simply set the price for each edge $e_i$ to be $p^*_i$.

Now consider the set of prices $p^*$. We show that, no matter in what order come the buyers, the final allocation is guaranteed to be $y^*$ with a proper tie-breaking policy. Thus the selling process always obtains welfare $\optwel$.
For every buyer $j$, consider the following two cases.
The first case is when $y^*_j=0$, from the constraint of (LP-Dual), $\sum_{i: e_i\in Q_j}p^*_i\geq v_j$. Since the seller has the power of tie-breaking, it can be guaranteed that buyer $j$ does not get any edge when she comes to the auction: Either she is not willing to buy the edge, or she is indifferent buying or not, but the seller chooses not to sell to her.

The second case is when $y^*_j=1$, from the above discussion, we must have $\sum_{i: e_i\in Q_j}p^*_i=v^*_j$. Now the seller chooses to sell the edges in $Q_j$ to buyer $j$.
It is immediate to verify that the above tie-breaking policy guarantees that the final allocation of this selling process is $y^*$, no matter in what order come the buyers. And the welfare of this selling process is $\optwel$. The set of prices $p^*$ can be computed in polynomial time by solving the dual LP.

\end{proof}
}


%In the rest of this section, we prove that a $\frac{2}{3}$-fraction of the optimal welfare can always be achieved via some pricing for any buyer profile. Both Example~\ref{example:path} and Theorem~\ref{thm:path_no_tie} imply that the tight ratio of path graph without the power of tie-breaking is $2/3$.

The main result in this section is the following theorem.

\begin{theorem}
\label{thm:path_no_tie}
There is an efficient algorithm, that, given any path graph $G$ and any buyer-profile $\fset=\set{(Q_j,v_j)}_{j\in [m]}$, computes a set of prices on edges of $G$ that achieves worst-case welfare at least $(2/3)\cdot \opt(G,\fset)$, without the power of tie-breaking.
\end{theorem}
\begin{proof}
%Without loss of generality we assume that the optimal solution $y^*$ covers the whole graph. Otherwise, 
%, since the price $\tilde p(Q_j)=+\infty$, which is above her value $v_j$. 
%Now the path graph is separated into disjoint intervals and we could apply the same argument for the sub-instance on every subpath.
From \Cref{thm:path}, (LP-Primal) has an integral optimal solution.  We denote by $y^*$ the integral optimal solution of (LP-Primal)  that maximizes $\sum_{j\in [m]}y^*_j$. Note that $y^*$ can be computed by solving a slightly different LP that is obtained from (LP-Primal) by changing its objective to $\sum_{j\in [m]}(v_j+\eps')\cdot y_j$, for some small enough $\eps'>0$.
Define $Y=\set{j\mid y^*_j=1}$ and
$\qset_Y=\set{Q_j\mid y^*_j=1}$. 
%\begin{proof}[Proof of Theorem~\ref{thm:path_no_tie}]
%Let $\qset_Y$ be a maximum-cardinality optimal integral solution. It can be computed efficiently via dynamic programming.
%\znote{need to explain how to find them efficiently} \ytnote{Maximum-cardinality solution can be found via dynamic program. An alternative way is to use the term ``maximal solution'' instead of ``maximum-solution'', and it would be easier to check.}

Define $\eps=\frac{1}{n^2}\cdot\min\set{v_j\mid j\in [m]}$.
We prove the following claim.
\begin{claim}
There is an optimal solution $p^*=(p^*(e))_{e\in E(G)}$ for (LP-Dual), such that 
(i) for each edge $e\in E(\qset_Y)$, $p^*(e)\geq \eps$; and (ii) 
for each $j\in [m]$, $p^*(Q_j)\geq v_j$.
\end{claim}
\begin{proof}
%Note that picking any optimal solution in (LP-Dual) can only guarantee non-negative prices. 
We construct another buyer-profile $\fset'$ from $\fset$ as follows. We add, for each $e\in E(G)$ a new buyer demanding the path consisting of a single edge $e$ with value $\eps$.
On one hand, it is easy to see that $y^*$ is still an optimal solution of this new instance. Let $p^*$ be any optimal solution for the correponding dual LP for the new instance. Clearly $p^*$ is also an optimal solution of (LP-Dual) and satisfies both properties. 
\end{proof}



We define $A=\set{j\mid v_j=p^*(Q_j)}$ and $\qset_A=\set{Q_j\mid j\in A}$.
%Recall that $\eps_1=\frac{1}{n^2}\cdot\min\set{v_j\mid j\in [m]}$. We further define $\eps_2=\frac{1}{n}\cdot\min\set{p^*(Q_j)-v_j\mid j\in [m]: p^*(Q_j)>v_j}$, and let $\eps=\min\{\eps_1,\eps_2\}$.
%\znote{to postpone}
%Notice that for every $j\in [m]$, $p^*(Q_j)\geq v_j$. 
%we are ensured that, no matter when she comes, she will not take the edges of $Q_j$ given the price vector $\tilde p$, as $v_j<\tilde p(Q_j)$.
%Let $\qset_A=\{Q_j\}_{j=1}^m$ be the set of all paths.
We say that a set $\qset\subseteq \qset_A$ of edge-disjoint paths is \emph{good}, iff set $\qset_A\setminus \qset$ does not contain another subset $\qset'$ of $|\qset'|\ge 2$ edge-disjoint paths, such that
%$|\qset'|\geq 2$ if $|\qset|\geq 2$ and 
$\bigcup_{Q_j\in \qset'}Q_j=\bigcup_{Q_j\in \qset}Q_j$. %and (3) $\sum_{Q_j\in \qset'}v_j\geq\sum_{Q_j\in \qset}v_j$
%In other words, there does not exist another way of covering the subpath $I$ using set of paths in $\qset_A$.
%with $|\qset|\geq 2$, we say that $\qset$ satisfies the \emph{covering property} if and only if there does not exist a set $\qset'\subseteq (\qset_A\setminus \qset)$ of paths that satisfies (i) $|\qset'|\ge 2$; (ii) the paths in $\qset'$ are edge-disjoint; and (iii) $\bigcup_{Q\in \qset'}Q=\bigcup_{Q\in \qset}Q$. We say any single path ($|\qset|=1$) satisfies the covering property.
%there exists a subset $\qset'\subseteq \qset_A\setminus \qset$ of edge-disjoint paths such that $\bigcup_{Q\in \qset}Q=\bigcup_{Q\in \qset'}Q$.
We use the following lemma.



%\begin{proposition}
%For any set of edge-disjoint paths $\qset$, let $\qset=\bigcup_{i=1}^k\qset_i$ where any two set of paths $\qset_i$ and $\qset_j$ do not share the same endpoint. Then $\qset$ satisfies the covering property if and only if $\qset_i$ satisfies the covering property for all $i$.
%\end{proposition}


\begin{lemma}\label{claim:covering_implies_optimal}
There is an efficient algorithm, that, given a good set $\qset$ of edge-disjoint paths, computes a set of positive prices $p=\{p(e)\}_{e\in E(\qset)}$%that always guarantees to 
that achieves worst-case welfare at least $\sum_{Q_j\in \qset}v_j$.% and satisfies that, for each edge $e\in E(\qset)$, $|p(e)-p^*(e)|<\eps$.
%For any set of edge-disjoint paths $\qset^*\subseteq \qset_A$ that satisfies the covering property, there exists a non-negative price vector $\tilde p$, that guarantees to achieve welfare $v(\qset^*)$. %that is equal to the total welfare of $\qset^*$.
%Moreover, such a vector can be computed in polynomial time. %\todo{To argue this when the prices must be non-negative.}
\end{lemma}
\begin{proof}
%\ytnote{Actually, from the following proof, we only need the theorem in a special case. That is, suppose that the optimal allocation is two connected paths. If there are no other way of partitioning the entire path, then there exists an item pricing that sells all items without tie-breaking.}{\color{red}To check. }
%We consider only selling edges in the subpath $I$.
We denote $I=\bigcup_{Q_j\in \qset}Q_j$ and $\qset_I=\{Q_j\in \qset_A\mid Q_j\subseteq I\}$. 
First, for each edge $e\notin E(I)$, we set its price $p(e)=+\infty$. 
Therefore, all buyers $j$ with $Q_j\notin \qset_I$ cannot get her demand path.
We will show that we can efficiently compute prices $\set{p(e)}_{e\in E(I)}$ for edges of $I$, such that (i) for each path $Q_j\in \qset$, $v_j>p(Q_j)$; and (ii) for each path $Q_j\in \qset_I\setminus \qset$, $v_j<p(Q_j)$. %Note that any buyer $j\not\in A$ will never be served under price vector $p$. Thus for any agent's order, all buyers $j$ where $Q_j\in\qset$ can get her demand path and thus the welfare is at least $\sum_{Q_j\in \qset}v_j$.    
It is clear that the set $\set{p(e)}_{e\in E(G)}$ of prices achieves worst-case welfare $\sum_{Q_j\in \qset}v_j$.

The existence of prices $\set{p(e)}_{e\in E(I)}$ is equivalent to the feasibility of the following system.
\begin{equation}\label{lp:covering-primal}
\left\{
\begin{array}{cccc}
\displaystyle \sum_{e\in Q_j}p(e) &< & v_j,&\forall Q_j\in\qset;\\
\displaystyle \sum_{e\in Q_j}p(e) & >& v_j,&\forall Q_j\in \qset_I\setminus \qset.
\end{array}
\right.
\end{equation}
From the definition of $A$, and since $\qset_I\subseteq\qset_A$, for each path $Q_j\in \qset_I$, $\sum_{e\in Q_j}p^*(e)= v_j$. 
We denote $\alpha(e)=p(e)-p^*(e)$ for all $e\in E(I)$, then system~\eqref{lp:covering-primal} is feasible if the following system is feasible, for some small enough $\eps'>0$.
\begin{equation}\label{lp:covering-primal2}
\left\{
\begin{array}{cccc}
\displaystyle \sum_{e\in Q_j}\alpha(e) &\le & -\eps',&\forall Q_j\in\qset;\\
\displaystyle \sum_{e\in Q_j}\alpha(e) & \ge & \eps',&\forall Q_j\in \qset_I\setminus \qset.
\end{array}
\right.
\end{equation}
%Take $\sigma>0$ to be a sufficiently small constant. 
%such that $\eps<2^{-poly(B)}$ where $B$ is the bit-complexity of the input. 
\iffalse
Then system~\eqref{lp:covering-primal2} is feasible if and only if the following system is feasible, for a small enough constant $\sigma>0$.
\begin{equation}\label{lp:covering-primal3}
\left\{
\begin{array}{cccc}
\displaystyle \sum_{e\in Q_j}\alpha(e) &\le & -\sigma,&\forall Q_j\in\qset;\\
\displaystyle \sum_{e\in Q_j}-\alpha(e) & \leq & -\sigma,&\forall Q_j\in \qset_I\setminus \qset.
\end{array}
\right.
\end{equation}
\fi
From Farkas' Lemma,
%\footnote{We note that Farkas' Lemma works for systems with only non-strict inequalities, but it can be easily adapted here to work with systems with strict inequalities. The additional constraints $\beta_j\le 1, \forall Q_j\in \qset_I$ will not influence the feasibility of the system due to scaling.}
system~\eqref{lp:covering-primal2} is feasible if and only if the following system is infeasible.
\begin{equation}\label{lp:covering-dual}
\left\{
\begin{array}{rccc}
\displaystyle \sum_{Q_j\in \qset}\beta_j\cdot\mathbbm{1}[e\in Q_j]-\sum_{Q_j\in \qset_I\setminus \qset}\beta_j\cdot\mathbbm{1}[e\in Q_j] &=& 0,&\forall e\in E(I);\\
\displaystyle\sum_{Q_j\in \qset_I}\beta_j&>& 0;\\
\beta_j & \in & [0,1],&\forall Q_j\in \qset_I.
\end{array}
\right.
\end{equation}
where the additional constraints $\beta_j\le 1, \forall Q_j\in \qset_I$ will not influence the feasibility of the system due to scaling.
By similar arguments in the proof of \Cref{lem:primal-tu}, we can show that the coefficient matrix in system \eqref{lp:covering-dual} is totally unimodular. Therefore, system \eqref{lp:covering-dual} is feasible iff it admits an integral solution.
\iffalse
\begin{lemma}\label{lem:covering-integral-solu}
System~\eqref{lp:covering-dual} is feasible if and only if it admits an integral solution.
\end{lemma}
\begin{proof}
We prove that the coefficient matrix $C$ in system \eqref{lp:covering-dual} is totally unimodular. Similar to the proof of Theorem~\ref{lem:primal-tu}, for any set of rows $R=\{i_1,i_2,\cdots,i_k\}$ such that $i_1<i_2<\cdots<i_k$, We define the partition $R_1=\{i_1,i_3,i_5,...\}$ be the set with odd index and $R_2=\{i_2,i_4,i_6,...\}$ be the set with even index. For every column $j$, $Q_j$ is an subpath and thus the ones (or -1s for $Q_j\in \qset_I\setminus \qset$) in the vector $(C_{ij})_{i=1}^n$ are consecutive. Hence the difference between $\sum_{i\in R_1}C_{ij}$ and $\sum_{i\in R_2}C_{ij}$ is at most 1. By Lemma~\ref{lem:proposition-tu}, $C$ is totally unimodular.
%we can partition the set of rows to two sets $I_1=\{i_1,i_3,i_5,\cdots\}$ and $I_2=\{i_2,i_4,i_6,\cdots\}$, such that the sum of coefficients of $\beta_j$ in two sets differ by at most 1 for every $j$. 
\end{proof}
%Thus, \eqref{lp:covering-dual} is feasible if and only if it admits an integral solution.
\fi
Assume for contradiction that  \eqref{lp:covering-dual} is feasible, let $\beta^*\in \set{0,1}^{\qset_I}$ be an integral solution of \eqref{lp:covering-dual}.
Note that the constraints 
$\sum_{Q_j\in \qset}\beta^*_j\cdot\mathbbm{1}[e\in Q_j]-\sum_{Q_j\in \qset_I\setminus \qset}\beta^*_j\cdot\mathbbm{1}[e\in Q_j] = 0,\forall e\in E(I)$ and the fact that paths of $\qset$ are edge-disjoint
imply that the paths in set $\qset'=\{Q_j\mid \beta_j=1\}$ are edge-disjoint. Note that $\qset'\cap\qset=\emptyset$ and $\bigcup_{Q_j\in \qset'}Q_j=\bigcup_{Q_j\in \qset}Q_j$, and this is a contradiction to the assumption that the set $\qset$ is good.
%Thus \eqref{lp:covering-dual} is infeasible as $Q^*$ satisfies the covering property. 
%Thus by Lemma~\ref{lem:covering-integral-solu} and the fact that $\qset$ is the good cover, system~\eqref{lp:covering-dual} is infeasible.
%Thus system \eqref{lp:covering-primal2} is feasible.
Therefore, system \eqref{lp:covering-dual} is infeasible, and system \eqref{lp:covering-primal2} is feasible.
%It follows that \eqref{lp:covering-primal} is feasible, and a positive solution can be computer efficiently using the Ellipsoid algorithm.
Let $(\alpha(e))_{e\in E(I)}$ be a solution of system~\eqref{lp:covering-primal2}, such that $\sum_{e\in E(I)} |\alpha(e)|\le \eps$. It is clear that such a solution exists due to scaling.
%Take any feasible solution $\alpha=\{\alpha_i\}_{i=1}^n\not= 0$ of system~\eqref{lp:covering-primal2}. Note that the vector $\alpha'$ where $\alpha'(e)=\frac{\eps}{2}\cdot\frac{\alpha(e)}{\max_e |\alpha(e)|},\forall e$ is also feasible. 
We set $p(e)=p^*(e)+\alpha(e)$ for all $e\in E(I)$, and it is clear that the set $\set{p(e)}_{e\in E(G)}$ of prices satisfies the property of \Cref{claim:covering_implies_optimal}.
Moreover, prices $\set{p(e)}_{e\in E(G)}$ are positive.
%and we can scale down $\alpha$ such that $p_i^*+\alpha\geq 0$ always holds for each $i$.
%\ytnote{Not very clear. Better way to say this?}
%Therefore system \eqref{lp:covering-primal} has integral feasible solution.
\end{proof}
%From the claim above, if there is no subset $\qset\subseteq (\qset_A\setminus \qset_Y)$ of paths satisfying the covering property, then we can efficiently compute a price vector $\tilde p$, such that the only buyers with $v_j>\tilde p(Q_j)$ are the buyers that are assigned their demand paths in the optimal allocation. It follows that we can achieve revenue that is equal to the optimal welfare in this case.

% Assume that $\qset_Y$ is the maximum cardinality optimal solution. Let $\qset_R=\qset_A\setminus\qset_Y$ be the remaining paths that are not allocated in the optimal solution. It remains to consider the case where there is a subset $\qset\subseteq \qset_R$ of paths satisfying the covering property.

% For each path $Q_j\in\qset_Y$, let $T_j\subseteq \qset_R$ denote a set of paths such that
% \begin{itemize}
%     \item $Q_j\subseteq\bigcup_{Q\in T_j} Q$;
%     \item There exists a subset $\qset\subseteq \qset_Y$ of paths in the optimal solution, such that $\bigcup_{Q\in T_j} Q=\bigcup_{Q\in \qset_Y} Q$;
%     \item $T_j$ has maximum cardinality. Furthermore, $|\bigcup_{Q\in T_j} Q|$ is the largest among every possible max-cardinality $T_j$.
% \end{itemize}
% In other words, $T_j$ not only covers $Q_j$, but also exactly covers some contiguous paths in $\qset_Y$.

% Let $\qset_Y^1\subseteq \qset_Y$ be the set of paths $Q_j$ that do not have corresponding $T_j$; $\qset_Y^2=\qset_Y\setminus\qset_Y^1$ be the rest of them.
% Let $\tset^*$ be the set of $T_j$ such that each item that is contained in one of the paths in $\qset_Y^2$ is covered at least once and at most twice by paths in $\tset^*$. {\color{red} Add explanation or trivial?} Let $\qset_Y^3\subseteq \qset_Y^2$ be a minimal subset of paths in $\qset_Y^2$ such that each item in $\qset_Y^2$ is covered exactly twice by paths in $\tset^*\cup \qset_Y^3$. {\color{red} Add explanation or trivial?}

% Consider multi-set of paths $\tset=\tset^*\cup \qset_Y^3\cup \qset^1\cup\qset^1$. Each item sold in the optimal solution $\qset_Y$ is covered exactly 2 times in $\tset$. If we can divide $\tset$ into three sets of paths, such that each set of paths satisfy the covering property, then there exists one set of paths that can obtain pricing revenue that is $2/3$ of optimal welfare.
% Now we will show how to make the division via the following coloring procedure.

% Suppose that $\tset^*\cup \qset_Y^3$ covers $k$ disjoint paths $I_1,I_2,\cdots,I_k$. Fix a particular path $I_a$.
% For all paths in $\tset^*\cup \qset_Y^3$ that is contained in $I_a$, we will use three colors to color them, such that
% \begin{enumerate}
%     \item No two paths with same color contains the same item;
%     \item No three contiguous paths have the same color;
%     \item For each endpoint shared by at most three paths, all of the paths are colored differently;
%     \item For an endpoint shared by 4 paths, all three colors are used to color these paths, and two paths with the same color are
%     \begin{enumerate}
%         \item both from $\qset_Y^3$, or
%         \item both from an path $T_j\in\tset^*$, or
%         \item both from $\qset_Y^1$, or
%         \item from $\qset_Y^1$ and from an path $T_j\in\tset^*$ respectively.
%     \end{enumerate}
% \end{enumerate}
% Such coloring exists by greedily coloring all paths from left to right. Then paths of each color are formed by two connected paths in $\tset$, or single paths in $\tset$ that do not share endpoints. Since the single paths

We now complete the proof of Theorem~\ref{thm:path_no_tie} using \Cref{claim:covering_implies_optimal}. 
%We will construct a price vector $\tilde p$, such that for each $i\in [n]$, $|\tilde p(e_i)-p^*(e_i)|<\eps$. Thus $\tilde p(e_i)>0$ for every $i$. Also it is immediate to verify that, for each buyer $j$, if $v_j<p^*(Q_j)$, then $v_j<\tilde p(Q_j)$; and if $v_j>p^*(Q_j)$, then $v_j>\tilde p(Q_j)$.Then, for any buyer $j\not\in A$, she will never be served as $v_j<\tilde p(Q_j)$. 


%We construct prices $\tilde p=(\tilde p(e))_{e\in E(G)}$ based on $p^*$ and $y^*$, as follows. 
We denote $\qset_Y=\set{Q_1,Q_2,\ldots,Q_k}$, where the paths are indexed according to the order in which they appear on $G$.
First, for each edge $e\notin E(\qset_Y)$, we set its price $\tilde p(e)=+\infty$.
%In other words, if an edge $e$ is not assigned to any buyer in the optimal allocation $y^*$, then we do not intend to sell it. 
Therefore, any buyer $j$ with $e\in Q_j$ cannot take her demand path.
In fact, we may assume without loss of generality that $\bigcup_{1\le j\le k}Q_j=G$, since otherwise we can view each connected component (which is also a path) of graph $\bigcup_{1\le j\le k}Q_j$ as the whole graph, and compute prices for its edges separately.
%Let $G_Y$ be the graph obtained by taking the union of all paths of $\qset_Y$. It is clear that $G_Y$ is the union

%Each item sold in the optimal solution $\qset_Y$ is covered exactly 2 times in $\qset^*$. 
We will compute three sets $\hat\qset_1,\hat\qset_2,\hat\qset_3\subseteq \qset_A$ of edge-disjoint paths, such that 
%(i) the paths in each of $\hat\qset_1,\hat\qset_2,\hat\qset_3$ are edge-disjoint;
\begin{enumerate}
\item every edge of $E(G)$ is contained in exactly two paths of $\hat\qset_1,\hat\qset_2,\hat\qset_3$; and
\item \label{prop: good_cover} for each $t\in \set{1,2,3}$, if we further partition the set $\hat\qset_t$ into subsets $\hat\qset^1_t,\ldots,\hat\qset^{r_t}_t$, such the union of the paths in each set $\hat\qset^1_t$ forms a connected component (which is also a path) of graph $\bigcup_{Q_j\in \hat\qset_t}Q_j$, then each of the sets $\hat\qset^1_t,\ldots,\hat\qset^{r_t}_t$ is a good set of edge-disjoint paths. 
\end{enumerate}
By definition, $\sum_{Q_j\in \hat\qset_1}v_j+\sum_{Q_j\in \hat\qset_2}v_j+\sum_{Q_j\in \hat\qset_3}v_j=2\cdot\opt(G,\fset)$.
Assume without loss of generality that $\sum_{Q_j\in \hat\qset_1}v_j\ge (2/3)\cdot\opt(G,\fset)$.
Then from Lemma~\ref{claim:covering_implies_optimal}, there exist prices $\set{\tilde p(e)}_{e\in E(\qset_Y)}$ that achieves worst-case welfare at least $\sum_{Q_j\in \hat\qset_1}v_j\ge (2/3)\cdot\opt(G,\fset)$.

\paragraph{Compute the sets $\hat\qset_1,\hat\qset_2,\hat\qset_3$.}
We now compute the desired sets $\hat\qset_1,\hat\qset_2,\hat\qset_3$ of edge-disjoint paths, which, from the above discussion, completes the proof of Theorem~\ref{thm:path_no_tie}.


We start by defining $\hat\qset$ to be the multi-set that contains, for each path $Q_j\in\qset_Y$, two copies $Q'_j,Q''_j$ of $Q_j$. 
%We define $\hat\qset$ to be the multi-set of paths that contains, for each path $Q_j\in\qset_Y$, two copies $Q^1_j,Q^2_j$ of $Q_j$. 
We initially set
\begin{itemize}
\item $\hat\qset_1=\set{Q'_{6r+3},Q'_{6r+4}\mid 1\le r\le k/6} \cup\set{Q''_{6r},Q''_{6r+1}\mid 1\le r\le k/6}$;
\item $\hat\qset_2=\set{Q'_{6r+1},Q'_{6r+2}\mid 1\le r\le k/6} \cup\set{Q''_{6r+4},Q''_{6r+5}\mid 1\le r\le k/6}$; and
\item $\hat\qset_3=\set{Q'_{6r+2},Q'_{6r+3}\mid 1\le r\le k/6} \cup\set{Q''_{6r+2},Q''_{6r+3}\mid 1\le r\le k/6}$.
\end{itemize}
See Figure~\ref{fig:path-1} for an illustration.
Clearly, sets $\hat\qset_1,\hat\qset_2,\hat\qset_3$ partition $\hat\qset$, each contains edge-disjoint paths, and every edge appears twice in paths of $\hat\qset_1,\hat\qset_2,\hat\qset_3$.
However, sets $\hat\qset_1,\hat\qset_2,\hat\qset_3$ may not satisfy Property~\ref{prop: good_cover}.
We will then iteratively modify sets $\hat\qset_1,\hat\qset_2,\hat\qset_3$, such that at the end Property~\ref{prop: good_cover} is satisfied.

Throughout, we also maintain graphs $G_t=\bigcup_{Q\in \hat{\qset}_t}Q$, for each $t\in \set{1,2,3}$. As sets $\hat\qset_1,\hat\qset_2,\hat\qset_3$ change, graphs $G_1,G_2,G_3$ evolve.
We start by scanning the path $G$ from left to right, and process, for each each connected component of graphs $G_1,G_2,G_3$, as follows.

%while always ensuring that each set of $\hat\qset_1,\hat\qset_2,\hat\qset_3$ contains edge-disjoint paths, and every edge appears twice in paths of $\hat\qset_1\cup\hat\qset_2\cup\hat\qset_3$.

%For convenience, we sometimes say that we label path $Q_j$ by $t$ for some $t\in \set{1,2,3}$ 
%Now we will show how to make the division via the following coloring procedure. The illustration is shown in Figure~\ref{fig:path-coloring}. First color the paths in $\qset^*$ using 3 colors, such that the coloring satisfy the following ``good'' properties:
%For convenience, we denote by $v_i$ the vertex shared by path $Q_j,Q_{j+1}$, for each $1\le j\le k-1$, so path $Q_j$ has endpoints $v_{j-1},v_{j}$.
\iffalse
\begin{enumerate}
    \item No two paths with same color share the same edge;
    \item No three contiguous paths have the same color;
    \item For each endpoint shared by at most three paths, all of the paths are colored differently;
    %\mingfeinote{Every edge in $\qset_Y$ is copied twice. Aren't each endpoint is shared by 2 or 4 paths?} \ytnote{I want to define this good property, to be still feasible after the first step.}
    \item For each endpoint shared by 4 paths, all three colors are used to color these paths, and two paths with the same color are
    \begin{enumerate}
        \item both from $\qset_Y$, or
        \item both from $\qset'_Y:=\qset^*\setminus\qset_Y$, the second copy of the optimal solution.
    \end{enumerate}
\end{enumerate}
Such coloring is guaranteed to exist. In fact, for every $Q_j\in \qset_Y$, let $g(Q_j)=j\text{ mod }6$. For every $Q_j'\in \qset_Y'$, let $g(Q_j')=(j+3)\text{ mod }6$. We color a path blue if its $g$-value is 0 or 1, red if its $g$-value is 2 or 3, and green if its $g$-value is 4 or 5. One can easily verify that the above coloring satisfies all the properties.
\fi


%An example is shown in Figure~\ref{fig:path-1}. Then paths of each color are formed by two connected paths in $\tset$, or single paths in $\tset$ that do not share endpoints. %Since by Lemma~\ref{claim:covering_implies_optimal} all single paths satisfy the covering property, 
We first process the connected component in $G_1$ formed by the single path $Q_1''$. Clearly, set $\set{Q_1''}$ is good, since if there are other paths $\hat Q,\hat Q'\in \qset_A$ such that $\hat Q,\hat Q'$ are edge-disjoint and $\hat Q\cup \hat Q'=Q_1$, then the set $\set{\hat Q,\hat Q',Q_2,\ldots,Q_k}$ corresponds to another integral optimal solution $\hat y^*$ of (LP-Primal) with $\sum_{j\in [m]}\hat y^*_j=k+1>k=\sum_{j\in [m]}\hat y^*_j$, a contradiction to the definition of $y^*$. We do not modify path $Q''_1$ in $\hat{\qset}_1$ and continue to the next iteration.

%Note that any single path here must be the good cover, since otherwise there exists a set of paths with size at least 2 that covers the same subpath, which violates the fact that $\qset_Y$ has the maximum cardinality among all optimal solution. 

%Thus we are interested in the connected paths. They may not be the good cover, but we may manipulate set $\qset^*$ as follows to make them become the good cover.


We then process the connected component in $G_2$ formed by the paths $Q_1',Q_2'$. If the set $\set{Q_1',Q_2'}$ is good, then we do not modify this component and continue to the next iteration. Assume now that the set $\set{Q_1',Q_2'}$ is not good.
From similar arguments, there exist two other paths $Q^*_1,Q^*_2\in \qset_A$, such that $Q^*_1,Q^*_2$ are edge-disjoint and $Q^*_1\cup Q^*_2=Q_1\cup Q_2$. %It cannot be the case that $Q_1$ or $Q_2$ can be exactly covered by multiple paths in $\qset_A$, or $Q_1\cup Q_2$ can be exactly covered by at least 3 paths in $\qset_A$, since $\qset_Y$ has maximum cardinality.
We then replace the paths $Q'_1,Q'_2$ in $\hat{\qset}_2$ by paths $Q^*_1,Q^*_2$.
Let $v^*_1$ be the vertex shared by paths $Q^*_1,Q^*_2$, so $v^*_1\ne v_1$. We distinguish between the following cases.

\textbf{Case 1. $v^*_1$ is to the left of $v_1$ on path $G$.}
As shown in Figure~\ref{fig:path-2}, we keep the path $Q^*_2$ in $\hat{\qset}_2$, and move path $Q^*_1$ to $\hat{\qset}_3$.
Clearly, we create two new connected components: one in $G_3$ formed by a single path $Q^*_1$, and the other in $G_2$ formed by a single path $Q^*_2$.
From similar arguments, the corresponding singleton sets $\set{Q^*_1}, \set{Q^*_2}$ are good.

\textbf{Case 2. $v^*_1$ is to the right of $v_1$ on path $G$.}
As shown in Figure~\ref{fig:path-4}, we keep the path $Q^*_2$ in $\hat{\qset}_2$, move path $Q^*_1$ to $\hat{\qset}_1$ and additionally move the path $Q'_1$ processed in previous iteration to $\hat{\qset}_2$.
Clearly, we create two new connected components: one in $G_1$ formed by a single path $Q^*_1$, and the other in $G_2$ formed by a single path $Q^*_2$.
From similar arguments, the corresponding singleton sets $\set{Q^*_1}, \set{Q^*_2}$ are good. 
Note that we have additionally moved $Q'_1$ to $\hat{\qset}_2$, but since we did not change the corresponding component, the singleton set $\set{Q'_1}$ is still good.

\begin{figure}[h]
\centering
\subfigure[An illustration of paths in set $\hat{\qset}_1\cup \hat{\qset}_2\cup \hat{\qset}_3$ at the beginning.]{\scalebox{0.4}{\includegraphics{interval_1.jpg}}\label{fig:path-1}}
\subfigure[An illustration of path modification in Case 1.]{\scalebox{0.4}{\includegraphics{interval_2.jpg}}\label{fig:path-2}}
\subfigure[An illustration of path modification in Case 2.]{\scalebox{0.4}{\includegraphics{interval_4.jpg}}\label{fig:path-4}}
\subfigure[How old and new paths/components may possibly interact.]{\scalebox{0.39}{\includegraphics{interval_3.jpg}}\label{fig:path-3}}
\caption{Illustrations of the algorithm for computing path sets $\hat{\qset}_1,\hat{\qset}_2,\hat{\qset}_3$.}
\end{figure}
%This procedure can be done repeatedly, and each time the number of unmarked endpoints adjacent to 4 paths reduce by 1. Finally, the number of unmarked endpoints adjacent to 4 paths become 0, which means that paths of each color is composed by disjoint single paths or two connected paths which are the good cover. Thus there must exist paths of one color whose total value is at least $2/3$ of the optimal welfare.

We continue processing the remaining connected components in the same way until all components are good. We will show that, every time a connected component is not good and the corresponding two paths are replaced with two new paths, the connected components in $G_1,G_2,G_3$ that we have processed in previous iterations will stay good. Therefore, the algorithm will end up producing good components in $G_1,G_2,G_3$ consisting of a good set of one or two edge-disjoint paths.

To see why this is true, consider an iteration where we are processing a component consisting of paths $Q''_i, Q''_{i+1}$, and there exists edge-disjoint paths $Q^*_i,Q^*_{i+1}$ such that $Q^*_i\cup Q^*_{i+1}=Q''_i\cup Q''_{i+1}$, while the endpoint $v^*_i$ shared by $Q^*_i$ and $Q^*_{i+1}$ is an endpoint of a processed component, as shown in Figure~\ref{fig:path-3}. 
Note that this is the only possibility that the new components may influence the previous components,
However, we will show that this is impossible. 
Note that $Q''_{i}\in \qset_Y$. 
We denote by $Q^r$ the path with endpoints $v^*_i$ and $v_i$, then clearly paths $Q^*_i, Q^r$ are not in $\qset_Y$, edge-disjoint and satisfy that $Q_{i}=Q^*_i\cup Q^r$.
Consider now the set $(\qset_Y\setminus \set{Q_{i}})\cup \set{Q^*_i, Q^r}$. It is clear that this set corresponds to another integral optimal solution $\hat y^*$ of (LP-Primal) with $\sum_{j\in [m]}\hat y^*_j=k+1>k=\sum_{j\in [m]}\hat y^*_j$, a contradiction to the definition of $y^*$.
\end{proof}


We complement \Cref{thm:path_no_tie} with the following theorem.

\begin{theorem}\label{thm:path_no_tie_hardness}
\label{thm: path_no_tie_lower_bound}
There exists a path graph $G$ and a buyer-profile $\fset$, such that any set of prices on edges of $G$ can achieve worst-case revenue at most $(2/3)\cdot \opt(G,\fset)$, without the power of tie-breaking.
\end{theorem}
\begin{proof}
Let $G$ be a path consisting of three edges $e_1,e_2,e_3$, that appears on the path in this order. The buyer-profile is described below.
%Table~\ref{table:example_path}.
\begin{itemize}
\item Buyer $B_1$ demands the path consisting of a single edge $e_1$, with value $1$;
\item Buyer $B_2$ demands the path consisting of a single edge $e_3$, with value $1$;
\item Buyer $B_3$ demands the path consisting of edges $e_1,e_2$, with value $2$; and
\item Buyer $B_4$ demands the path consisting of edges $e_2,e_3$, with value $2$.
\end{itemize}

\iffalse
\begin{table}[H]
\centering
		\begin{tabular}{ c|c|c}
			Buyer & Demand & Value \\
			\hline
			$B_1$ & $e_1$ & 1 \\
			\hline
			$B_2$ & $e_3$ & 1 \\
			\hline
			$B_3$ & $e_1,e_2$ & 2\\
			\hline
			$B_4$ & $e_2,e_3$ & 2
		\end{tabular}
		\label{table:example_path}
		\caption{Example for Path Graph}
	\end{table}
\fi
	
It is clear that the optimal allocation is assigining the $e_1$ to $B_1$ and $e_2,e_3$ to $B_4$ (or assigning $e_3$ to $B_2$ and $e_1,e_2$ to buyer $B_3$), and the optimal welfare is $\opt(G,\fset)=3$.
We now show that, for any prices $p(e_1),p(e_2),p(e_3)$ on edges $e_1,e_2,e_3$, there is an order of the four buyers, such that, if the buyers come in this order and make decisions with the power of tie-breaking, the resulting welfare is at most $2$. 
Note that this completes the proof of \Cref{thm: path_no_tie_lower_bound}.

%Thus any pricing can only guarantee welfare at most $(2/3)\cdot \opt(G,\fset)$.
	%{\color{red} Todo}
We distinguish between different cases.

\textbf{Case 1. $p(e_1)\leq 1$ and $p(e_3)\leq 1$.} We let buyers $B_1$ and $B_2$ come first and take edges $e_1$ and $e_3$, respectively (note that the seller does not have the power of tie-breaking, so buyers can decide whether or not to take their path when the price equals their value). Now buyers $B_3, B_4$ cannot get their paths, so the resulting welfare is $2$.

%\textbf{Case 2. $p(e_1)=1$ or $p(e_3)=1$.} We let buyers $B_1$ and $B_2$ come first, and let them \textbf{not} take edges $e_1$ or $e_3$. Now the demand of buyer $B_3$ and $B_4$ can not be fulfilled anymore and thus the total welfare is 2. 

\textbf{Case 2. $p(e_1)>1$ or $p(e_3)>1$.} Assume without loss of generality that $p(e_1)>1$. If $p(e_2)+p(e_3)\leq 2$, then we let buyer $B_4$ come first and take edges $e_2$ and $e_3$. It is clear that no other buyer can get her path, so the resulting welfare is 2. If $p(e_2)+p(e_3)>2$, so $p(e_1)+p(e_2)+p(e_3)>3$. Note that it is impossible in this case all edges are sold. Therefore, the resulting welfare is at most $2$.
\end{proof}




==> plan.tex <==

\begin{itemize}
    \item Focus on no tie-breaking for the whole paper.
    \item Mention previous results with tie-breaking: 1 for path, 3/2 for tree. \mingfeinote{Do we need a proof for tree?}
    \item (1) Path: 3/2
    \item (2) Tree: O(1). Only mention tree in the intro. In proof sketch, say that we obtain the result by studying star/spider.
    \item (3) General Graph: Both upper and lower bound. \mingfeinote{See if we can change the upper bound proof (Theorem~\ref{thm:general_graph}) to no tie-breaking.} Say that the lower bound works even if we have tie-breaking.
    \item (4) Resource Augmentation.
\end{itemize}

==> sec5.1.tex <==
\subsection{Path}\label{sec:pathnt}

We first focus on the case when $G$ is a single path. Unlike the scenario with tie-breaking power, where the optimal welfare can be obtained with some set of prices (Theorem~\ref{thm:path}), the competitive ratio may be strictly larger than 1 when the seller has no tie-breaking power.

\begin{theorem}\label{thm:path_no_tie_hardness}
\label{thm: path_no_tie_lower_bound}
$\rationt(\pathh)\geq 3/2$, i.e. there exists a path graph $G$ and an instance $\fset$, such that any set of prices achieves worst-case welfare at most $2/3\cdot \opt(G,\fset)$, when the seller has no tie-breaking power.
\end{theorem}

In Theorem~\ref{thm:path_no_tie} we prove that the competitive ratio $3/2$ is tight for path graphs, when the seller has no tie-breaking power.

\begin{theorem}
\label{thm:path_no_tie}
$\rationt(\pathh)\leq 3/2$. Moreover, the prices that achieve the competitive ratio 3/2 can be computed efficiently.
%There is an efficient algorithm, that, given any path graph $G$ and any buyer-profile $\fset=\set{(Q_j,v_j)}_{j\in [m]}$, computes a set of prices on edges of $G$ that achieves worst-case welfare at least $(2/3)\cdot \opt(G,\fset)$, without the power of tie-breaking.
\end{theorem}
%\begin{proof}
%Without loss of generality we assume that the optimal solution $y^*$ covers the whole graph. Otherwise,
%, since the price $\tilde p(Q_j)=+\infty$, which is above her value $v_j$.
%Now the path graph is separated into disjoint intervals and we could apply the same argument for the sub-instance on every subpath.
Before giving a proof sketch of Theorem~\ref{thm:path_no_tie}, we first present some definitions and lemmas required in the proof. From \Cref{thm:path}, (LP-Primal) has an integral optimal solution.  We denote by $y^*$ the integral optimal solution of (LP-Primal)  that maximizes $\sum_{j\in [m]}y^*_j$. Note that $y^*$ can be computed by solving a slightly different LP that is obtained from (LP-Primal) by changing its objective to $\sum_{j\in [m]}(v_j+\eps')\cdot y_j$, for some small enough $\eps'>0$.
Define $Y=\set{j\mid y^*_j=1}$ and
$\qset_Y=\set{Q_j\mid y^*_j=1}$.

\begin{lemma}\label{lem:price-strictly-positive}
There is an $\eps>0$ and an optimal solution $\set{p^*(e)}_{e\in E(G)}$ for (LP-Dual), such that
(i) for each edge $e\in E(\qset_Y)$, $p^*(e)\geq \eps$; and (ii)
for each $j\in [m]$, either $p^*(Q_j)=v_j$, or $p^*(Q_j)>v_j+n\eps$.
\end{lemma}

Now choose $\eps>0$ and the prices $p^*$ from Lemma~\ref{lem:price-strictly-positive}. We define $A=\set{j\mid v_j=p^*(Q_j)}$ and $\qset_A=\set{Q_j\mid j\in A}$.
%Recall that $\eps_1=\frac{1}{n^2}\cdot\min\set{v_j\mid j\in [m]}$. We further define $\eps_2=\frac{1}{n}\cdot\min\set{p^*(Q_j)-v_j\mid j\in [m]: p^*(Q_j)>v_j}$, and let $\eps=\min\{\eps_1,\eps_2\}$.
%\znote{to postpone}
%Notice that for every $j\in [m]$, $p^*(Q_j)\geq v_j$.
%we are ensured that, no matter when she comes, she will not take the edges of $Q_j$ given the price vector $\tilde p$, as $v_j<\tilde p(Q_j)$.
%Let $\qset_A=\{Q_j\}_{j=1}^m$ be the set of all paths.
\begin{definition}
We say that a set $\qset\subseteq \qset_A$ of edge-disjoint paths is \emph{good}, iff set $\qset_A\setminus \qset$ does not contain another subset $\qset'$ of $|\qset'|\ge 2$ edge-disjoint paths, such that
%$|\qset'|\geq 2$ if $|\qset|\geq 2$ and
$\bigcup_{j:Q_j\in \qset'}Q_j=\bigcup_{j:Q_j\in \qset}Q_j$. %and (3) $\sum_{Q_j\in \qset'}v_j\geq\sum_{Q_j\in \qset}v_j$
%In other words, there does not exist another way of covering the subpath $I$ using set of paths in $\qset_A$.
%with $|\qset|\geq 2$, we say that $\qset$ satisfies the \emph{covering property} if and only if there does not exist a set $\qset'\subseteq (\qset_A\setminus \qset)$ of paths that satisfies (i) $|\qset'|\ge 2$; (ii) the paths in $\qset'$ are edge-disjoint; and (iii) $\bigcup_{Q\in \qset'}Q=\bigcup_{Q\in \qset}Q$. We say any single path ($|\qset|=1$) satisfies the covering property.
%there exists a subset $\qset'\subseteq \qset_A\setminus \qset$ of edge-disjoint paths such that $\bigcup_{Q\in \qset}Q=\bigcup_{Q\in \qset'}Q$.
\end{definition}

We prove the following lemma about good edge-disjoint paths.


%\begin{proposition}
%For any set of edge-disjoint paths $\qset$, let $\qset=\bigcup_{i=1}^k\qset_i$ where any two set of paths $\qset_i$ and $\qset_j$ do not share the same endpoint. Then $\qset$ satisfies the covering property if and only if $\qset_i$ satisfies the covering property for all $i$.
%\end{proposition}


\begin{lemma}\label{claim:covering_implies_optimal}
There is an efficient algorithm that, given a good set $\qset$ of edge-disjoint paths, computes a set of positive prices $p=\{p(e)\}_{e\in E(G)}$%that always guarantees to
that achieves worst-case welfare at least $\sum_{Q_j\in \qset}v_j$.% and satisfies that, for each edge $e\in E(\qset)$, $|p(e)-p^*(e)|<\eps$.
%For any set of edge-disjoint paths $\qset^*\subseteq \qset_A$ that satisfies the covering property, there exists a non-negative price vector $\tilde p$, that guarantees to achieve welfare $v(\qset^*)$. %that is equal to the total welfare of $\qset^*$.
%Moreover, such a vector can be computed in polynomial time. %\todo{To argue this when the prices must be non-negative.}
\end{lemma}




%From the claim above, if there is no subset $\qset\subseteq (\qset_A\setminus \qset_Y)$ of paths satisfying the covering property, then we can efficiently compute a price vector $\tilde p$, such that the only buyers with $v_j>\tilde p(Q_j)$ are the buyers that are assigned their demand paths in the optimal allocation. It follows that we can achieve revenue that is equal to the optimal welfare in this case.

% Assume that $\qset_Y$ is the maximum cardinality optimal solution. Let $\qset_R=\qset_A\setminus\qset_Y$ be the remaining paths that are not allocated in the optimal solution. It remains to consider the case where there is a subset $\qset\subseteq \qset_R$ of paths satisfying the covering property.

% For each path $Q_j\in\qset_Y$, let $T_j\subseteq \qset_R$ denote a set of paths such that
% \begin{itemize}
%     \item $Q_j\subseteq\bigcup_{Q\in T_j} Q$;
%     \item There exists a subset $\qset\subseteq \qset_Y$ of paths in the optimal solution, such that $\bigcup_{Q\in T_j} Q=\bigcup_{Q\in \qset_Y} Q$;
%     \item $T_j$ has maximum cardinality. Furthermore, $|\bigcup_{Q\in T_j} Q|$ is the largest among every possible max-cardinality $T_j$.
% \end{itemize}
% In other words, $T_j$ not only covers $Q_j$, but also exactly covers some contiguous paths in $\qset_Y$.

% Let $\qset_Y^1\subseteq \qset_Y$ be the set of paths $Q_j$ that do not have corresponding $T_j$; $\qset_Y^2=\qset_Y\setminus\qset_Y^1$ be the rest of them.
% Let $\tset^*$ be the set of $T_j$ such that each item that is contained in one of the paths in $\qset_Y^2$ is covered at least once and at most twice by paths in $\tset^*$. {\color{red} Add explanation or trivial?} Let $\qset_Y^3\subseteq \qset_Y^2$ be a minimal subset of paths in $\qset_Y^2$ such that each item in $\qset_Y^2$ is covered exactly twice by paths in $\tset^*\cup \qset_Y^3$. {\color{red} Add explanation or trivial?}

% Consider multi-set of paths $\tset=\tset^*\cup \qset_Y^3\cup \qset^1\cup\qset^1$. Each item sold in the optimal solution $\qset_Y$ is covered exactly 2 times in $\tset$. If we can divide $\tset$ into three sets of paths, such that each set of paths satisfy the covering property, then there exists one set of paths that can obtain pricing revenue that is $2/3$ of optimal welfare.
% Now we will show how to make the division via the following coloring procedure.

% Suppose that $\tset^*\cup \qset_Y^3$ covers $k$ disjoint paths $I_1,I_2,\cdots,I_k$. Fix a particular path $I_a$.
% For all paths in $\tset^*\cup \qset_Y^3$ that is contained in $I_a$, we will use three colors to color them, such that
% \begin{enumerate}
%     \item No two paths with same color contains the same item;
%     \item No three contiguous paths have the same color;
%     \item For each endpoint shared by at most three paths, all of the paths are colored differently;
%     \item For an endpoint shared by 4 paths, all three colors are used to color these paths, and two paths with the same color are
%     \begin{enumerate}
%         \item both from $\qset_Y^3$, or
%         \item both from an path $T_j\in\tset^*$, or
%         \item both from $\qset_Y^1$, or
%         \item from $\qset_Y^1$ and from an path $T_j\in\tset^*$ respectively.
%     \end{enumerate}
% \end{enumerate}
% Such coloring exists by greedily coloring all paths from left to right. Then paths of each color are formed by two connected paths in $\tset$, or single paths in $\tset$ that do not share endpoints. Since the single paths

Now we are ready to sketch the proof of \Cref{thm:path_no_tie}. We will prove Theorem~\ref{thm:path_no_tie} using \Cref{claim:covering_implies_optimal}.
%We will construct a price vector $\tilde p$, such that for each $i\in [n]$, $|\tilde p(e_i)-p^*(e_i)|<\eps$. Thus $\tilde p(e_i)>0$ for every $i$. Also it is immediate to verify that, for each buyer $j$, if $v_j<p^*(Q_j)$, then $v_j<\tilde p(Q_j)$; and if $v_j>p^*(Q_j)$, then $v_j>\tilde p(Q_j)$.Then, for any buyer $j\not\in A$, she will never be served as $v_j<\tilde p(Q_j)$.
%We construct prices $\tilde p=(\tilde p(e))_{e\in E(G)}$ based on $p^*$ and $y^*$, as follows.
We denote $\qset_Y=\set{Q_1,Q_2,\ldots,Q_k}$, where the paths are indexed according to the order in which they appear on $G$.
First, for each edge $e\notin E(\qset_Y)$, we set its price $\tilde p(e)=+\infty$.
%In other words, if an edge $e$ is not assigned to any buyer in the optimal allocation $y^*$, then we do not intend to sell it.
Therefore, any buyer $j$ with $e\in Q_j$ cannot take her demand path.
In fact, we may assume without loss of generality that $\bigcup_{1\le j\le k}Q_j=G$, since otherwise we can view each connected component (which is also a path) of graph $\bigcup_{1\le j\le k}Q_j$ as the whole graph, and compute prices for its edges separately.
%Let $G_Y$ be the graph obtained by taking the union of all paths of $\qset_Y$. It is clear that $G_Y$ is the union

%Each item sold in the optimal solution $\qset_Y$ is covered exactly 2 times in $\qset^*$.
The crucial step of the proof is to compute three sets $\hat\qset_1,\hat\qset_2,\hat\qset_3\subseteq \qset_A$ of edge-disjoint paths, such that
%(i) the paths in each of $\hat\qset_1,\hat\qset_2,\hat\qset_3$ are edge-disjoint;
\begin{enumerate}
\item \label{prop: cover_twice} every edge of $E(G)$ is contained in exactly two paths of $\hat\qset_1,\hat\qset_2,\hat\qset_3$; and
\item \label{prop: good_cover} for each $t\in \set{1,2,3}$, consider every connected component in the graph generated from paths in $\hat\qset_t$. Then set of paths in every connected component is a good set of edge-disjoint paths.
%if we further partition the set $\hat\qset_t$ into subsets $\hat\qset^1_t,\ldots,\hat\qset^{r_t}_t$, such the union of the paths in each set $\hat\qset^1_t$ forms a connected component (which is also a path) of graph $\bigcup_{Q_j\in \hat\qset_t}Q_j$, then each of the sets $\hat\qset^1_t,\ldots,\hat\qset^{r_t}_t$ is a good set of edge-disjoint paths.
\end{enumerate}
By property~\eqref{prop: cover_twice}, $\sum_{j:Q_j\in \hat\qset_1}v_j+\sum_{j:Q_j\in \hat\qset_2}v_j+\sum_{j:Q_j\in \hat\qset_3}v_j=2\cdot\opt(G,\fset)$.
Assume without loss of generality that $\sum_{j:Q_j\in \hat\qset_1}v_j\ge (2/3)\cdot\opt(G,\fset)$.
Then we can set prices $\set{\tilde p(e)}_{e\in E(\hat\qset_1)}$ according to Lemma~\ref{claim:covering_implies_optimal}, and $+\infty$ price for all other edges. By Lemma~\ref{claim:covering_implies_optimal}, the item pricing $\tilde p$ achieves worst-case welfare at least $\sum_{j:Q_j\in \hat\qset_1}v_j\ge (2/3)\cdot\opt(G,\fset)$.


==> special_graphs.tex <==
%\section{Competitive Ratio for Special Graphs}
\section{Warm Up: Competitive Ratio for Seller with Tie-breaking Power}
\label{sec:special_graph}
Throughout this section, we assume that the seller has tie-breaking power. 
In this section, we first analyze the competitive ratio when the underlying graph $G$ has special structures.
In Section~\ref{sec:no_tie_breaking}, we consider the case where the seller does not have tie-breaking power.

\subsection{Competitive Ratio for Path Graphs and Trees}
\label{subsec:path-tree}

Given any instance $\fset$, the hindsight optimal welfare is captured by an integer program. The relaxed linear program (LP-Primal) is shown in Equation~\eqref{equ:primal} in Section~\ref{subsec:result}. Its dual (LP-Dual) is shown in Equation~\eqref{equ:dual}.
We denote $\optlp(\qset, v)$ (or $\optlp$ if the instance is clear from context) the optimum of (LP-Primal). Clearly, $\optlp(\qset,v)\geq \opt(\qset, v)$. We first present a lemma that is useful throughout this section. The lemma shows that for any feasible integral solution achieved by rounding from the optimal fractional solution, we are able to compute prices to guarantee selling to the exact same set of buyers. 

\begin{lemma}\label{lem:rounding}
Let $y^*$ be any optimal solution of (LP-Primal) and let $y'\in \set{0,1}^n$ be any feasible integral solution of (LP-Primal), such that for each $j\in [n]$, $y'_j=0$ if $y_j^*=0$.
Then there exists a price vector $p=\set{p_i}_{i\in [m]}$ that achieves worst-case welfare $\sum_{j\in [n]}v_j\cdot y_j'$, if the seller has the power of tie-breaking. Moreover, the price vector $p$ can be computed efficiently. 
\end{lemma}

\begin{proof}
Let $p^*=\{p^*_i\}_{i\in [m]}$ be any optimal solution for (LP-Dual). 
We will show that, for any buyers' arrival order $\sigma$, with a proper tie-breaking rule, we can ensure with the prices $p^*$ that the outcome of the selling process is $y'$, and therefore it achieves welfare $\sum_{j\in [n]}v_j\cdot y_j'$.

Consider now a buyer $j$.
Assume first that $y_j'=0$, from the constraint of (LP-Dual), $\sum_{i\in Q_j}p^*_i\geq v_j$.
If $\sum_{i\in Q_j}p^*_i> v_j$, then the buyer $j$ cannot afford her demand set.
If $\sum_{i\in Q_j}p^*_i= v_j$, since the seller has the power of tie-breaking, the seller can choose not to give the demand set to her.
Assume now that $y_j'=1$, so $y_j^*>0$. From the complementary slackness, $\sum_{i \in Q_j}p^*_i=v_j$. The seller can sell the demand set $Q_j$ to buyer $j$.
Since $y'$ is a feasible solution of (LP-Primal), no items will be given to more than one buyer.
Moreover, it is easy to verify that the above tie-breaking rule ensures that this selling process's outcome is exactly $y'$, for any buyers' arrival order $\sigma$. Therefore, the worst-case welfare is $\sum_{j\in [n]}v_j\cdot y_j'$. The set of prices $p^*$ can be computed in polynomial time by solving the (LP-Dual).
\end{proof}

An immediate corollary of Lemma~\ref{lem:rounding} is for the highway problem, i.e. $G$ is a single path. In this case, there is always an integral optimal solution for (LP-Primal)~\cite{cheung2008approximation,schrijver1998theory}. Thus by Lemma~\ref{lem:rounding}, there exist prices that achieve worst-case welfare the same as optimal welfare.

\begin{theorem}
[\cite{cheung2008approximation,chawla2017stability}]
\label{thm:path}
$\ratio(\pathh)=1$.
\end{theorem}




==> spider.tex <==
\subsection{Spiders}\label{sec:spider}

\iffalse
\begin{theorem}
\label{thm:spider}
If we (the seller) has the power of tie-breaking (or not), then there is an efficient algorithm, that, given any buyer-profile $\set{(Q_j,v_j)}_{j\in [m]}$ in the spider graph, computes a set of prices $\set{p_e}_{e\in G}$ that achieves the revenue at least $1/3$ (or $\frac{2}{7}$) the optimal offline welfare.
\end{theorem}
\begin{proof}
We first find the optimal integral offline allocation that maximizes the total value. Consider an path composed by  $L=L_1\cup L_2$ two legs of the graph such that a path $Q=Q_1\cup Q_2$ is allocated on both legs in the offline allocation. Let $e_1\in Q_1\subseteq  L_1,e_2\in Q_2\subseteq L_2$ be the edges adjacent to the center. Denote by $\opt_{out}(L)$ be the total value of paths from $L\setminus Q$ in the optimal solution, in other words, the welfare contributed from edges unrelated to $Q$. Thus the optimal welfare from this leg is $\opt(L)=\opt_{out}(L)+v(Q)$. Denote by $\opt_{in}(L)$ be the optimal value of paths from $Q\setminus\{e_1,e_2\}$, in other words, the optimal welfare that can get collected from $Q$ that are unrelated to the center. $\opt_{in}(L)$ is a part of optimal offline allocation, but will appear in our later analysis.

Suppose that $\opt_{in}(L)=\delta v(Q)$. Clearly $\delta\leq 1$, since $\opt_{out}(L)+\opt_{in}(L)$ is also a feasible value of allocation on $L$, thus $\opt_{out}(L)+\opt_{in}(L)\leq \opt(L)=\opt_{out}(L)+v(Q)$.
Consider the following two pricing algorithms $p_L^1$ and $p_L^2$. 

Pricing $p_L^1$ set prices $p_L^1(e_1)=p_L^1(e_2)=\frac{1-\delta}{2}v(Q)$ to the edges connected to the center; for any edge $e\in Q\setminus\{e_1,e_2\}$, $p_L^1(e)$ equals the dual price in the LP solving $\opt_{in}(L)$ (when we do not have tie-breaking, add arbitrarily small $\eps$ to the price of edges in $Q\setminus\{e_1,e_2\}$ and reduce the price of edges $e_1$, $e_2$ such that $p_L^1(Q)=v(Q)$); for any edge $e\in L\setminus Q$, $p_L^1(e)=+\infty$. Notice that the buyer allocated path $Q$ in the optimal solution can still afford to purchase that path, since $p_L^1(Q)=2\cdot\frac{1-\delta}{2}v(Q)+\opt_{in}(L)=v(Q)$; any buyer purchasing $e_1$ or $e_2$ will contribute at least $\frac{1-\delta}{2}v(Q)$ to this leg $L$; any buyer that demands a path in $e\in Q\setminus\{e_1,e_2\}$ has value at most the price according to the discussion in Theorem~\ref{thm:path}, thus can be filtered out by tie-breaking (or additional price); any buyer that demands a path intersecting $L\setminus Q$ cannot afford to pay the infinite price. Thus the revenue $\rev(p_L^1)$ contributed to $L$ in pricing $p_L^1$ is at least $\frac{1-\delta}{2}v(Q)$.

Pricing $p_L^2$ set prices $p_L^2(e)$ for each edge $e\in L\setminus\{e_1,e_2\}$ to be the dual price in the LP solving the optimal welfare for $L\setminus\{e_1,e_2\}$; $p_L^2(e_1)=p_L^2(e_2)=+\infty$. The revenue contributed to $L$ in pricing $p_L^2$ is 
\begin{equation}\label{eqn:spider-pricing2}
    \rev(p_L^2)\geq\opt(L\setminus\{e_1,e_2\})\geq \opt_{in}(L)+\opt_{out}(L)=\delta v(Q)+\opt_{out}(L).
\end{equation}
Thus the better of the two item pricings grants revenue
\begin{eqnarray*}
    \max(\rev(p_L^1),\rev(p_L^2))&\geq& \frac{2}{3}\rev(p_L^1)+\frac{1}{3}\rev(p_L^2)\\
    &\geq&\frac{2}{3}\cdot\frac{1-\delta}{2}v(Q)+\frac{1}{3}(\delta v(Q)+\opt_{out}(L))\\
    &=&\frac{1}{3}(v(Q)+\opt_{out}(L))=\frac{1}{3}\opt(L).
\end{eqnarray*}
For each pair of legs such that a path is allocated in the optimal allocation, we run the better of the two pricings above. For a leg such that the paths allocated on it do not cross the center, the performance is only better. Such item pricing gives $\frac{1}{3}$-approximation to the optimal welfare.

For the case without tie-breaking, we have $\rev(p_L^2)\geq \frac{2}{3}(\delta v(Q)+\opt_{out}(L))$, thus $\max(\rev(p_L^1),\rev(p_L^2))\geq \frac{2}{7}\opt(L)$.

\end{proof}

\subsection{An improved approximation ratio for spiders}
\fi


%We show the following theorem that provides an improved tight competitive ratio for spider graphs when the seller has the power of tie-breaking.


In this section we consider the case where graph $G$ is a spider. The main result of this section is summarized in the following theorem.


\begin{theorem}
\label{thm:spiderimproved}
There is an efficient algorithm, that, given any spider graph $G$ and any buyer-profile $\fset=\set{(Q_j,v_j)}_{j\in [m]}$, computes a set of prices on edges of $G$ that achieves the worst-case revenue equal at least $(2/3)\cdot\opt(G,\fset)$, with the power of tie-breaking.
\end{theorem}

The remainder of this section is dedicated to the proof of Theorem~\ref{thm:spiderimproved}.
Similarly as in the proof of Theorem~\ref{thm:star2}, we consider the linear program (LP-Primal). We use the following lemma, whose proof is similar to that of Lemma~\ref{lem:matching-half-integral} and is deferred to Section~\ref{sec: Proof of spider-half-integral}.

\begin{lemma}\label{lem:spider-half-integral} 
If $G$ is a spider graph, then (LP-Primal) has a half-integral optimal solution $y^*$. Moreover, such a solution can be computed efficiently.
\end{lemma}

Denote by $\optlp$ the optimal value of (LP-Primal), and let $y^*$ be a half-integral optimal solution of (LP-Primal) given by Lemma~\ref{lem:spider-half-integral}. 
Denote $J_{1/2}=\set{j\mid y^*_j=1/2}$ and $J_1=\set{j\mid y^*_j=1}$.
Clearly, paths of $\set{Q_j\mid j\in J_{1}}$ are edge-disjoint, and they are also edge-disjoint from paths of $\set{Q_j\mid j\in J_{1/2}}$.
We will show that we can efficiently compute a subset $J'\subseteq J_{1/2}$, such that (i) the paths of $\set{Q_j\mid j\in J'}$ are edge-disjoint; and (ii) the total value of paths in $\set{Q_j\mid j\in J'}$ is at least $\frac{1}{3}\cdot \sum_{j\in J_{1/2}}v_j$.
We claim that this implies Theorem~\ref{thm:spiderimproved}. To see why this is true, consider (LP-Dual) and any optimal solution $p^*=\{p^*(e)\}_{e\in E(G)}$ of (LP-Dual), and then we simply set, for each edge $e\in E(G)$, its price to be $p^*(e)$. From strong duality and complementary slackness, for each $j\in J'\cup J_1$, $\sum_{i: e_i\in Q_j}p^*(e_i)=v_j$, and for each $j\notin J'\cup J_1$, $\sum_{i: e_i\in Q_j}p^*(e_i)\le v_j$. Therefore, we may apply the power of tie-breaking such that only buyers of $\set{B_j\mid j\in J'\cup J_1}$ may get their demand paths at price $p^*$, and this ensures that the revenue we obtain at the end of the algorithm is at least $\sum_{ j\in J'\cup J_1}v_j\ge \frac{2}{3}\cdot (\frac{1}{2}\cdot\sum_{j\in J_{1/2}}v_j+\sum_{j\in J_{1}}v_j)= \frac{2}{3}\cdot \optlp$.



It remains to show how to compute the subset $J'$ with desired properties. We use the following lemma.

\begin{lemma}\label{lem:tree-coloring}
Let $T$ be a tree, let $d\geq 2$ be an integer and let $\qset$ be a set of paths in $T$, such that every edge of $T$ appears in at most $d$ paths of $\qset$, then we can efficiently compute a partition of $\qset$ into $d+1$ subsets $\qset_1,\ldots,\qset_{d+1}$, such that for every $1\le i\le d+1$, paths in $\qset_i$ are edge-disjoint.
\end{lemma}

We provide the proof of Lemma~\ref{lem:tree-coloring} later, after we complete the proof of Theorem~\ref{thm:spiderimproved} using it.
Define $\qset=\set{Q_j\mid j\in J_{1/2}}$. Since $y^*$ is a feasible solution of (LP-Primal), $y^*_j=1/2$ for each $j\in J_{1/2}$ and $y^*_j=1$ for each $j\in J_{1}$, every edge of $G$ is contained in at most $2$ paths of $\qset$. Since $G$ is a spider graph, $G$ is also a tree.
From Lemma~\ref{lem:spider-half-integral}, we can efficiently obtain a partition $(\qset_1,\qset_2, \qset_3)$ of $\qset$, such that for each $1\le i\le 3$, paths in $\qset_i$ are edge-disjoint.
Therefore, at least one of sets $\qset_1,\qset_2,\qset_3$ contains edge-disjoint paths of total value at least $\frac{1}{3}\sum_{Q\in \qset}v(Q)=\frac{1}{3}\sum_{j\in J_{1/2}}v_j$. 
%This completes the proof of Theorem~\ref{thm:spiderimproved}.

We now show the proof of Lemma~\ref{lem:tree-coloring}.
\begin{proof}[Proof of Lemma~\ref{lem:tree-coloring}.]
We construct an algorithm that partitions the set $\qset$ of paths into $d+1$ subsets $\qset_1,\ldots,\qset_{d+1}$.
We root $T$ at an arbitrarily chosen vertex $r\in V(T)$, and we say that a vertex $v\in V(T)$ is \emph{at the $i$-th level} iff the tree-distance between $v$ and $r$ in $T$ is $i$.
The algorithm will compute the sets $\qset_1,\ldots,\qset_{d+1}$ iteratively.
Initially, all sets are set to be $\emptyset$.
The algorithm proceeds sequentially in phases. In the $i$-th phase, the algorithm process all vertices at the $i$-th level one-by-one. 
Upon processing a vertex $v$, we will assign all paths  containing at least one edge of $E_v$ to some set of $\set{\qset_1,\ldots,\qset_{d+1}}$, where $E_v$ is the set of edges connecting $v$ to some of its children.

Fix an integer $i$ and a vertex $v$ at the $i$-th level, and we now describe the iteration of processing the vertex $v$. Let $\qset(v)$ contain all paths of $\qset$ that contains at least one edge connecting $v$ to some of its children.
The $\qset(v)$ can be partitioned into three subsets:
set $\qset^0(v)$ contains all paths of $\qset(v)$ that are already assigned to some set of $\set{\qset_1,\ldots,\qset_{d+1}}$;
set $\qset^1(v)$ contains all paths of $\qset(v)$ that are not yet already assigned and contains exactly $1$ edge of $E_v$; and
set $\qset^2(v)$ contains all paths of $\qset(v)$ that are not yet already assigned and contains exactly $2$ edges of $E_v$.
Note that each path of $\qset^0(v)$ must contain the edge $\hat e$ connecting $v$ to its parent vertex and exactly one edge of $E_v$, so they must belong to distinct sets of $\set{\qset_1,\ldots,\qset_{d+1}}$.
We construct an auxiliary graph $H$ as follows.
The vertex set is $V(H)=\set{u_{\hat e}}\cup \set{u_e\mid e\in E_v}\cup \set{\hat u_Q\mid Q\in \qset^1(v)}$. The edge set is partitioned into three subsets $E(H)=E_0\cup E_1\cup E_2$, where 
$E_0=\set{(u_e,v)\mid Q\in \qset^0(v), e= Q\cap E_v}$, $E_1=\set{(u_e,\hat u_Q)\mid Q\in \qset^1(v), e= Q\cap E_v}$, and
$E_2=\set{(u_e,u_{e'})\mid Q\in \qset^2(v), \set{e,e'}= Q\cap E_v}$.
Clearly, every path of $\qset(v)$ correspond to an edge in $E(H)$, that we denote by $f_Q$. 
It is clear from the definition of $H$ that, for every pair $Q,Q'$ of paths in $\qset(v)$, $Q$ and $Q'$ are edge-disjoint iff edges $f_{Q}$ and $f_{Q'}$ of $E(H)$ do not share a vertex.

Since every edge $e\in E_v$ is contained in at most $d$ paths of $\qset(v)$, from the definition of graph $H$, every vertex in $H$ has degree at most $d$. 
From Vizing's Theorem~\cite{vizing1964estimate,misra1992constructive}, we can efficiently find a coloring of all edges of $E(H)$ with $d+1$ colors, such that edges with same color do not share vertices.
Note that, since all edges in $\set{f_Q\mid \qset^{0}(v)}$ share the vertex $u_{\hat e}$, these edges will have different colors in any valid edge-coloring. 
We now assign, for each $Q\in \qset^{0}(v)$, all paths $Q'$ of $\qset(v)$ whose corresponding edge $f_{Q'}\in \qset(v)$ has the same color as edge $f_Q$, to the same set of $\set{\qset_1,\ldots,\qset_{d+1}}$.
And then we assign, for any color that is not used by edges in $\set{f_Q\mid Q\in \qset^{0}(v)}$, all paths whose corresponding edge $f_{Q'}\in \qset(v)$ has this color to a distinct set of $\set{\qset_1,\ldots,\qset_{d+1}}$ that does not contain paths of $ \qset^{0}(v)$.
This completes the iteration of processing the vertex $v$.
Since edges of have different colors, it is clear that, after this iteration, each set of $\set{\qset_1,\ldots,\qset_{d+1}}$ contains edge-disjoint paths.
Therefore, if we keep processing all vertices in this way, then we obtain a valid partition of the original set $\qset$ of paths into at most $d+1$ subsets $\qset_1,\ldots,\qset_{d+1}$, such that the paths in each subset are edge-disjoint.
\end{proof}


We also study the case where the seller does not have the power of tie-breaking.

\begin{theorem}\label{thm:spider-no-tiebreak}
For any constant $\eps>0$, there is an efficient algorithm, that, given any spider graph $G$ and any buyer-profile $\fset=\set{(Q_j,v_j)}_{j\in [m]}$, computes a set of prices on edges of $G$ that achieves the worst-case revenue equal at least $(\frac{2}{7}-\eps)\cdot\opt(G,\fset)$, without the power of tie-breaking.
\end{theorem}

\begin{proof}
Let $\qset$ be the set of paths in the optimal allocation. 
We define $\qset_1$ to be the set of all paths in $\qset$ that contains the center of the spider, and we define $\qset_2=\qset\setminus \qset_1$. For each path $Q\in \qset_1$, we define $G_Q$ to be the graph obtained by taking the union of all (one or two) legs whose edge sets intersect with $E(Q)$, and we denote $E_Q=E(G_Q)$. Then $E(G)=\bigcup_{Q\in \qset_1}E_Q$, and $\opt(G,\fset)=\sum_{Q\in\qset_1}\opt(G_Q,\fset)$.

Let $e_{Q,1}$ (and possibly $e_{Q,2}$) be the one (or two) edges that are in Q and has the spider center as one endpoint.
Define $G'_Q$ to be the graph with edge set $E'_Q=\{e|e\in E_Q\setminus Q\}$; in other words, $G'_Q$ contains all edges not in $Q$ but in $E_Q$, and $G''_Q$ contains all. Then $\opt(G_Q,\fset)=\opt(G'_Q,\fset)+v(Q)$. Define $G''_Q$ to be the graph with edge set $E''_Q=Q\setminus\{e_{Q,1},e_{Q,2}\}$; in other words, $G''_Q$ is the graph formed edges in $Q$, but excluding the center of the spider. 

Let $\alpha_Q=\frac{\opt(G''_Q,\fset)}{v(Q)}$. Clearly $\alpha_Q\leq 1$, since $E''_Q\subseteq Q$. The item pricing $p$ we construct sets one of the following two item pricings $p_1$ and $p_2$ on $E_Q$.
\begin{enumerate}
	\item For each $e\in E'_Q$, $p_1(e)>\opt(G,\fset)$ is large enough to prevent anyone from buying it; for each $e\in E''_Q$, $p_1(e)=p^*(e)+\frac{1}{n}\eps$, where $p^*$ is the dual prices $p$ from Theorem~\ref{thm:path} on $G''_Q$ with welfare $\opt(G''_Q,\fset)$; for each $e=e_{Q,1}$ or $e_{Q,2}$, $p_1(e)=\frac{(1-\alpha_Q)v(Q)}{2}-\eps$. Then no buyer demanding a path containing an edge in $E'_Q$ can afford to pay her path. Also since the utility of any buyer in $\fset$ is at most 0 in $p^*$, thus no buyer demanding a path with only edges in $E''_Q$ can afford to purchase her path. Also since the total price of edges in $Q$ is $\sum_{e\in E''_Q}p_1(e)+p_1(e_{Q,1})+p_1(e_{Q,2})<\opt(G''_Q,\fset)+\eps+(1-\alpha_Q)v(Q)-2\eps<v(Q)$, thus the buyer with demand $Q$ has positive utility for purchasing her path. Therefore, if item pricing $p$ sets $p_1$ for edges in $E_Q$, at least one of $e_{Q,1}$ and $e_{Q,2}$ is sold under $p$, which contributes $\frac{(1-\alpha_Q)v(Q)}{2}-\frac{1}{n}\eps$ revenue from edges in $E_Q$.
	\item For each $e\in E'_Q\cup E''_Q$, $p_2(e)$ is the price of edge $e$ by applying Theorem~\ref{thm:path_no_tie} to $G'_Q\cup G''_Q$, which is a union of at most two path graphs; for each $e=e_{Q,1}$ or $e_{Q,2}$, $p_2(e)>\opt(G,\fset)$ is large enough to prevent anyone from buying it. Then if item pricing $p$ sets $p_2$ for edges in $E_Q$, the total revenue from the two legs is at least $\frac{2}{3}\opt(G'_Q\cup G''_Q,\fset)\geq \frac{2}{3}\opt(G'_Q,\fset)+\frac{2}{3}\opt(G''_Q,\fset)=\frac{2}{3}\opt(G'_Q,\fset)+\frac{2}{3}\alpha_Qv(Q)$. 
\end{enumerate}
Let item pricing $p$ sets prices $p_1$ on $E_Q$ if $\frac{(1-\alpha_Q)v(Q)}{2}-\eps>\frac{2}{3}\opt(G'_Q,\fset)+\frac{2}{3}\alpha_Qv(Q)$, and sets prices $p_1$ on $E_Q$ otherwise. Then the revenue of $p$ is lower bounded by
\begin{eqnarray*}
& &\sum_{Q\in \qset_1}\max\left(\frac{(1-\alpha)v(Q)}{2}-\eps,\frac{2}{3}\opt(G'_Q,\fset)+\frac{2}{3}\alpha_Qv(Q)\right)\\
&\geq&\sum_{Q\in \qset_1}\frac{4}{7}\left(\frac{(1-\alpha)v(Q)}{2}-\eps\right)+\frac{3}{7}\left(\frac{2}{3}\opt(G'_Q,\fset)+\frac{2}{3}\alpha_Qv(Q)\right)\\
&=&\sum_{Q\in \qset_1}\left(\frac{2}{7}v(Q)+\frac{2}{7}\opt(G'_Q,\fset)-\frac{4}{7}\eps\right)\\
&=&\sum_{Q\in \qset_1}\left(\frac{2}{7}\opt(G_Q,\fset)-\frac{4}{7}\eps\right)>\frac{2}{7}\opt(G,\fset)-\frac{4n}{7}\eps.
\end{eqnarray*}
The theorem is proved by scaling $\eps$ properly.
\end{proof}






\subsubsection{Proof of Lemma~\ref{lem:spider-half-integral}}
\label{sec: Proof of spider-half-integral}

In this section we provide the proof of Lemma~\ref{lem:spider-half-integral}, using Lemma~\ref{lem:matching-half-integral}. 

We first modify the buyer profile as follows. For each edge $e$ of $G$, we add a buyer $B_e$ who demands the path that contains a single edge $e$ and has value $0$ upon the path. Equivalently, we consider the following linear program.
\begin{eqnarray*}
	\mbox{(LP-1)}	&\text{maximize } 
	\sum_{j\in [m]}v_j\cdot y_j\\
	\mbox{s.t.}
	& \hat y_i+\sum_{j: e_i\in Q_j}y_j= 1&\forall\text{ }1\le i\le n\\
	& y_j\ge 0&\forall\text{ } j\in [m]\\
	& \hat y_i\ge 0&\forall\text{ } 1\le i\le n
\end{eqnarray*}
It is easy to see that (LP-1) is equivalent to (LP-Primal), in the sense that (i) their optimal values are the same; and (ii) any optimal solution to (LP-1) naturally induces an optimal solution to (LP-Primal), and vice versa.
Consider now an optimal solution $y^*=(y^*_j)_{j\in [m]}$ of (LP-Primal). We define $\hat y^*\in [0,1]^n$ as: for each $1\le i\le n$, $\hat y^*_i=1- \sum_{j: e_i\in Q_j}y^*_j$. It is easy to see that $(y^*,\hat y^*)$ is an optimal solution of (LP-1).

We will now construct a star graph $H$ and a buyer profile $\fset'$ on $H$ as follows. Assume that the spider graph $G$ contains $\ell$ legs, and the $k$-th leg is denoted by $L_k$ (so $E(G)=\bigcup_{1\le k\le \ell}E(L_k)$).
Then $H$ is a star graph with $\ell$ edges, that are denoted by $\tilde e_{1}, \tilde e_2,\ldots,\tilde e_{\ell}$, respectively.
We now construct the buyer profile $\fset'$ iteratively.
Denote $\qset=\set{Q_1,\ldots,Q_m}\cup \set{(e_i)\mid e_i\in E(G)}$.
Throughout, we maintain: (i) for each path $Q\in \qset$, a real number $x_Q$, that is initialized as follows: if $Q=Q_j$ for some $j\in [m]$, then $x_Q=y^*_j$; if $Q=(e_i)$ for some $e_i\in E(G)$, then $x_Q=\hat y^*_i$; and
(ii) a buyer profile $\fset'$, that initially contains no buyers.
In each iteration, we will add one buyer into $\fset'$ and modify the values $\set{x_Q}_{q\in \qset}$. We will maintain the invariant that for each $1\le k\le \ell$, the sum $Z_e=\sum_{Q: e\in Q}x_Q$ are the same for all edges $e\in E_k$ of the $k$-th leg are the same (but the sums $Z_e,Z_{e'}$ may be distinct for edges $e,e'$ that belong to distinct legs). Clearly, initially this invariant holds.
We now describe an iteration. Let $\hat Q=\arg_{Q\in \qset: x_Q\ne 0}\min\set{x_Q}$.
We consider the following two cases.

\textbf{Case 1. Path $\hat Q$ contains edges from two distinct legs.} Assume path $\hat Q$ contains some edges from $L_{k_1},L_{k_2}$. Let $P_1$ be the subpath of $L_{k_1}$ formed by edges of $L_{k_1}\setminus \hat Q$, and we define $P_2$ similarly. We denote by $v_1,v'_1$ the endpoints of $P_1$, where $v'_1$ is the leaf of the leg $L_{k_1}$. We use the following claim.

\begin{claim}
\label{clm: extending path}
If $P_1\ne \emptyset$, then there exists an path $Q\in \qset$, such that (i) $x_Q\ge x_{\hat Q}$; and (ii) $Q$ is a subpath of $P_1$ and contains $v_1$ as one of its endpoints.
\end{claim}
\begin{proof}
Denote by $\hat e,\hat e'$ the edges incident to $v_1$, where $\hat e$ belongs to $\hat Q$ and $\hat e'$ belongs to $P_1$. 
Assume for contradiction that there is no such $Q$, then any path $Q\in \qset$ with $x_Q>0$ that contains  edge $\hat e'$ must also contain edge $\hat e$. However, since edges $\hat e,\hat e'$ belong to the same leg, and the path $\hat Q$ contains $\hat e$ but not $\hat e'$, the invariant that $Z_{\hat e}=Z_{\hat e'}$ cannot hold, a contradiction.
\end{proof}

As an easy corollary of Claim~\ref{clm: extending path}, we can find a set $\qset'_1\subseteq \qset$ of paths, such that (i) the paths of $\qset'_1$ are edge-disjoint; (ii) the union of paths of $\qset'_1$ is $P_1$; and (iii) for each $Q\in \qset'_1$, the value $x_Q\ge x_{\hat Q}>0$.
Similarly, we can find a set $\qset'_2\subseteq \qset$ of paths, such that (i) the paths of $\qset'_2$ are edge-disjoint; (ii) the union of paths of $\qset'_2$ is $P_2$; and (iii) for each $Q\in \qset'_2$, the value $x_Q\ge x_{\hat Q}>0$.
Therefore, if we set $\qset'=\set{\hat Q}\cup \qset'_1\cup \qset'_2$, then the paths of $\qset'$ are edge-disjoint, their union is $L_{k_1}\cup L_{k_2}$, and for each path $Q\in \qset'$, $x_Q\ge x_{\hat Q}$.
We then add a buyer to $\fset'$ as follows. Its demand path $P$ contains two edges $\tilde e_{k_1}, \tilde e_{k_1}$, and its value is defined as $v(P)=\sum_{Q\in \qset'}v(Q)$.
We also define $w^*_P=x_{\hat Q}$, and then we decrease the value $x_Q$ for all $Q\in \qset'$ by $x_{\hat Q}$.

\textbf{Case 2. Path $\hat Q$ contains edges from one leg.} Assume path $\hat Q$ contains only edges of $L_{k_1}$. We define path $P_1$ similarly as in Case 1. Via similar arguments, we can compute a set $\qset'_1$ of edge-disjoint paths whose union is $P_1$, and $x_Q\ge x_{\hat Q}> 0$ for each path $Q\in \qset'_1$.
We denote by $v_2$ the endpoint of $\hat Q$ that is closer to the center of the spider. 
If $v_2$ is the center then we set $\qset'_2=\emptyset$.
Otherwise, by repeatedly applying Claim~\ref{clm: extending path} to the subpath of $L_{k_1}$ between $v_2$ and the center (that we denote by $P_2$), we can compute a set $\qset'_2$ of edge-disjoint paths with $x_Q\ge x_{\hat Q}> 0$ for each path $Q\in \qset'_2$, such that the union of paths of $\qset'_2$ is either $P_2$ or the union of $P_2$ with some other entire leg $L_{k_2}$. 
Assume the former, then we add a buyer to $\fset'$ as follows. Its demand path $P$ contains one edge $\tilde e_{k_1}$, and its value is defined as $v(P)=\sum_{Q\in \qset'}v(Q)$, where $\qset'=\set{\hat Q}\cup \qset'_1\cup \qset'_2$.
Assume the latter, then we add a buyer to $\fset'$ as follows. Its demand path $P$ contains two edges $\tilde e_{k_1},e_{k_2}$, and its value is defined as $v(P)=\sum_{Q\in \qset'}v(Q)$.
In both cases, we also define $w^*_P=x_{\hat Q}$, and then we decrease the value $x_Q$ for all $Q\in \qset'$ by $x_{\hat Q}$.
We say that paths in $\qset'$ \emph{contributes} to path $P$. 


This finishes the description of an iteration.
Clearly, after each iteration, the invariant that for each $1\le k\le \ell$, the sum $Z_e$ are the same for all edges $e\in E_k$ of the $k$-th leg are the same still holds. Moreover, the number of paths $Q$ in $\qset$ with $x_Q>0$ is decreased by at least one after each iteration. Therefore, the algorithm terminates in $n+m$ iterations.
At the end, $x_Q=0$ for all paths $Q\in \qset$.
Let $\fset'=\set{(P,v_P)}_{P\in \pset}$ be the buyer profile that we get at the end of the algorithm. 
It is easy to see that (i) for each $j\in [m]$, $y^*_{j}=\sum_{P: Q_j\text{ contributes to }P}w^*_P$, and for each $1\le i\le n$, $\hat y^*_j=\sum_{P: (e_i)\text{ contributes to }P}w^*_P$; and (ii) $\sum_{P\in \pset}v_P\cdot w^*_P=\sum_{j\in [m]}v_j\cdot y^*_j$.
We consider the following linear program.
\begin{eqnarray*}
\mbox{(LP-2)}	&\text{maximize } 
\sum_{P\in \pset}v_P\cdot w_P\\
\mbox{s.t.}
& \sum_{P: \tilde e_i\in P}w_P= 1&\forall\text{ }1\le i\le \ell\\
& w_P\ge 0&\forall\text{ } P\le \pset
\end{eqnarray*}
We now show that $w^*=(w^*_P)_{P\in \pset}$ is an optimal solution of (LP-2). Assume the contrast that there exists another feasible solution $w'=(w'_P)_{P\in \pset}$ of (LP-2), such that $\sum_{P\in \pset}v_P\cdot w^*_P<\sum_{P\in \pset}v_P\cdot w'_P$.
We define vector $y'\in [0,1]^m$ as: for each $j\in [m]$, $y'_j=\sum_{P: Q_j\text{ contributes to }P}w'_P$, and define vector $\hat y'\in [0,1]^n$ as: for each $1\le i\le n$, $\hat y'_j=\sum_{P: (e_i)\text{ contributes to }P}w'_P$. It is easy to see that $(y',\hat y')$ is a feasible solution to (LP-1), and moreover, $\sum_{j\in [m]}v_j\cdot y'_j=\sum_{P\in \pset}v_P\cdot w'_P>\sum_{P\in \pset}v_P\cdot w^*_P=\sum_{j\in [m]}v_j\cdot y^*_j$. This causes a contradiction to the optimality of $(y^*,\hat y^*)$.
Therefore, from Lemma~\ref{lem:matching-half-integral}, $w^*$ is half-integral. Since for each $j\in [m]$, $y^*_{j}=\sum_{P: Q_j\text{ contributes to }P}w^*_P$, and for each $1\le i\le n$, $\hat y^*_j=\sum_{P: (e_i)\text{ contributes to }P}w^*_P$, $(y^*,\hat y^*)$ is also half-integral. It follows that $y^*$ is half-integral.



\iffalse
Without loss of generality the same as in the star case we assume each edge is fully allocated. Suppose that we can partition paths $Q_j$ with positive allocation $y_j^*$ into multiple groups $\qset_1,\qset_2,\cdots,\qset_s$ with allocation $z_1,z_2,\cdots,z_s$ respectively, such that
\begin{itemize}
    \item For each group $\qset_k$, the paths in it are edge-disjoint, and let $\cup\qset_k$ denote the union of the paths in $\qset_k$;
    \item For each group $\qset_k$, $\cup\qset_k$ is either a full leg of the spider, or two full legs of the spider;
    \item Each edge $e_i$ is allocated fractionally to exactly 1 group: $\sum_{j:e_i\in \qset_k}z_k=1$;
    \item Each path $Q_j$ has the same total weight in the groups as before: $\sum_{k:Q_j\in \qset_k}z_k=y^*_j$.
\end{itemize}
Then we can treat the graph as a star, and each group $\qset_k$ as a ``mega path'' $\cup\qset_k$ with allocation $z_k$ and value $\sum_{Q_j\in \qset_k}v_j$ and apply Lemma~\ref{lem:matching-half-integral} in the star case.

Now we show that such collection $\qset_1,\qset_2,\cdots,\qset_\ell$ of sets of paths always exists. In fact, we prove the following stronger lemma.

\begin{lemma}\label{lem:findpathinspider}
Let $\qset$ be a collection of paths $Q_j$ with allocation $y_j$, such that for each leg $L$ of the spider, any two edges have equal total allocation $y_L$. Formally, there exists a constant $y_L$ such that for any $e_i\in L$, $\sum_{Q_j\ni e_i}y_j=y_L$.
\end{lemma}
\begin{proof}[Proof of Lemma~\ref{lem:findpathinspider}]
When there is only one path $Q_j$ in $\qset$, we only need to define $Q_1$ to contain only this path with allocation $z_1=y^*_j$. If there are multiple paths in $\qset$, find a path $Q_j\in \qset$ with minimum allocation $y_j$. Construct $\qset_1=\{Q_j\}$, and we will add more paths to it later.

Assume that $Q_j$ is contained in leg $L$, the case where $Q_j$ is contained in two legs is exactly the same. We also assume that the edges in $L$ ordered from center are $e_1,e_2,\cdots,e_t$, and $Q_j=\{e_\ell,e_{\ell+1},\cdots,e_{r-1},e_r\}$. If $r\neq t$, then there must exist a path $Q$ starting at edge $e_{r+1}$ and ends at some edge $e_a$ such that $a\geq r+1$: otherwise, every path in $\qset$ containing $e_{r+1}$ must contain $e_r$, then the total weight of paths in $\qset$ containing $e_{r+1}$ is strictly less than the total weight of paths in $\qset$ containing $e_r$, which contradicts the assumption of the lemma. Let $Q=\{e_{r+1},e_{r+2},\cdots,e_{r'}\}$, and we add $Q$ to $\qset_1$. Repeatedly find path $Q$ that is connected to $\cup\qset_1$ and add $Q$ to $\qset_1$, until $e_t\in \cup\qset_1$. Similarly, we can grow $\qset_1$ from the other end $e_{\ell}$, until $\cup\qset_1$ ends at edge $e_1$ or the end of another leg $L'$. By this way we find a set of disjoint and connected paths $\qset_1$ that span exactly one or two legs of the graph. 
Figure~\ref{fig:spidertostar} gives an illustration of such expansion. 
\begin{figure}[h]
\centering
\includegraphics[width=0.9\columnwidth]{spidertostar.pdf}
\caption{Examples of the expansion of path $Q_1$ and $Q_2$. We find a sequence of paths including $Q_1$ that span exactly two legs, and a sequence of paths including $Q_2$ that span exactly one leg.\label{fig:spidertostar}}
\end{figure}
Let $z_1=y_j$, and set $y_{j'}\leftarrow y_{j'}-y_j$ for all $Q_{j'}\in \qset_1$. The remaining set of paths still satisfy the assumption of the lemma, and the above process reduces the total number of paths with positive allocation by at least 1. Thus repeatedly apply the above process and we can find the feasible groups of path sets. This finishes the proof of Lemma~\ref{lem:findpathinspider}, and Lemma~\ref{lem:spider-half-integral} suffices.
\end{proof}
\fi




\iffalse
\todo{the following theorem is currently false}

\begin{theorem}
If we (the seller) has the power of tie-breaking, then there is an efficient algorithm, that, given any buyer-profile $\set{(Q_j,v_j)}_{j\in [m]}$, computes a set of prices $\set{p_e}_{e\in G}$ that achieves the revenue equal to the optimal offline welfare.
\end{theorem}
\begin{proof}
Let $H'$ be a weighted graph defined as follows. The vertex set of $H'$ is $\set{u_i\mid e_i\in E(G)}$. The edge set of $H'$ is $\set{(u_i,u_{i'})\mid \exists j, Q_j=(e_i,e_{i'})}$, and the weight for the edge $(u_i,u_{i'})$ is set to be $v_j$, that we also denote by $v(i,i')$.
We augment $H'$ into another graph $H$ as follows. For each $1\le i\le L$, if there exists a buyer whose demand is the single edge $e_i$, then we add a new node $w_i$, and connect $w_i$ to $u_i$ via an edge, whose weight is set to be the value of this buyer on this single-edge path, that we denote by $v(i)$.
Therefore, there is an one-to-one correspondence between the buyers and the edges in $H$.

It is clear that an optimal (offline) allocation corresponds to an maximum weight matching in $H$. We compute an optimal matching $M$ in $H$. We will now show that there is a set of prices $\set{p_e}_{e\in G}$ on the edges of $G$, such that, no matter what order in which the buyers come, the selling process (with the seller having tie-breaking power) can lead to the optimal allocation corresponding to $M$, and achieves the revenue $\optwel$, the welfare of the allocation corresponding to $M$.


Consider the following feasibility linear program.
\begin{eqnarray*}
	\mbox{}	&\text{minimize } 0\\
	\mbox{s.t.}
	& p_i+p_{i'}\leq v(i,i') &\forall\text{ } e=(u_i,u_{i'})\in M\\
	& p_i\leq v(i) &\forall\text{ } e=(u_i,w_{i})\in M\\
	& p_i+p_{i'}\geq v(i,i') &\forall\text{ } e=(u_i,u_{i'})\in E(H)\setminus M\\
	& p_i\geq v(i) &\forall\text{ } e=(u_i,w_{i})\in E(H)\setminus M\\
	& p_i\ge 0&\forall\text{ } 1\le i\le L
\end{eqnarray*}
Assume that the above LP is infeasible, then there exist four sets $\set{\alpha(i,i')}_{(u_i,u_{i'})\in M}$, $\set{\beta(i)}_{(u_i,w_{i})\in M}$, $\set{\gamma(i,i')}_{(u_i,u_{i'})\in E(H)\setminus M}$, $\set{\theta(i)}_{(u_i,w_{i})\in E(H)\setminus M}$
of real numbers, such that:
\begin{eqnarray*}
%	\mbox{}	&\text{minimize } 0\\
%	\mbox{s.t.}
	& \sum_{i}\beta(i)v(i)+\sum_{(i,i')}\alpha(i,i')v(i,i')<\sum_{i}\theta(i)v(i)+\sum_{(i,i')}\gamma(i,i')v(i,i')\\
	& \beta(i)+\sum_{i':(u_i,u_{i'})\in M}\alpha(i,i')\geq  \theta(i)+\sum_{i':(u_i,u_{i'})\in E(H)\setminus M}\gamma(i,i') &\forall\text{ } 1\le i\le L\\
	& \alpha(i,i')\ge 0, \beta(i)\ge 0, \gamma(i,i')\ge 0, \theta(i)\ge 0&\forall\text{ } 1\le i,i'\le L
\end{eqnarray*}
{\color{red} Todo.}

\end{proof}
\fi


==> star.tex <==

\subsection{Stars}\label{sec:star}
In this section we consider the case where graph $G$ is a star, and we denote $E(G)=\set{e_1,\ldots,e_n}$. The main result of this section is summarized in the following theorem.

\begin{theorem}
\label{thm:star2}
There is an efficient algorithm, that, given any star graph $G$ and any buyer-profile $\fset=\set{(Q_j,v_j)}_{1\le j\le m}$, computes a set of prices on edges of $G$ that achieves the worst-case revenue equal at least $(2/3)\cdot\opt(G,\fset)$, with the power of tie-breaking.
\end{theorem}

\begin{proof}
\iffalse
Consider the following weighted graph $H$: For every edge $e_i$ in $G$, construct a node $a_i$ in $H$; For every buyer $j$, add a dummy node $b_j$ to $H$; For every buyer $j$, since $G$ is a star, her demand set $Q_j$ is of size at most 2. If $|Q_j|=2$, add edge $\hat{e}_j=(a_i,a_{i'})$ with weight $v_j$ to $H$ where $Q_j=\{e_i,e_{i'}\}$. Otherwise, add edge $\hat{e}_j=(a_i,b_j)$ with weight $v_j$ to $H$ where $Q_j=\{e_i\}$. Note that every buyer's demand now becomes an edge in graph $H$. Then the optimal offline welfare is equal to the total weight of maximum weight matching in $H$. (LP-Primal) describes the LP relaxation of a maximum weight matching problem. We have the following lemma.
\fi
Consider the following linear program.
\begin{eqnarray*}
	\mbox{(LP-Primal)}	&\text{maximize } 
	\sum_{1\le j\le m}v_j\cdot y_j\\
	\mbox{s.t.}
	&\sum_{j: e_i\in Q_j}y_j\leq 1&\forall\text{ }1\le i\le n\\
	& y_j\ge 0&\forall\text{ } 1\le j\le m
\end{eqnarray*}

The following lemma can be seen as a corollary of Claim 7 in~\cite{matchingLP}, which is probably a folklore result. For completeness, we provide its proof in Section~\ref{sec: proof of matching-half-integral}.
\begin{lemma}\label{lem:matching-half-integral}
If $G$ is a star graph, then (LP-Primal) is half-integral, and for each optimal solution $y^*\in \set{0,\frac 1 2,1}^{n}$, if we denote $J^*=\set{j\mid y^*_j=\frac{1}{2}}$ and define the graph $H$ as $V(H)=\set{u_i\mid e_i\in \bigcup_{j\in J^*}E(Q_j)}$ and $E(H)=\set{(u_i,u_{i'})\mid \exists j\in J^*, Q_j=(e_i,e_{i'})}$, then $H$ is the union of vertex-disjoint odd-length cycles.
\end{lemma}

Below is the Dual LP for (LP-Primal).
\begin{eqnarray*}
	\mbox{(LP-Dual)}	&\text{minimize } 
	\sum_{1\le i\le n}p(i)\\
	\mbox{s.t.}
	&\sum_{i: e_i\in Q_j}p(e_i)\geq v_j&\forall\text{ } 1\le j\le m\\
	& p(e_i)\ge 0&\forall\text{ } 1\le i\le n
\end{eqnarray*}
We denote by $\opt$ the optimal value of (LP-Primal), so $\opt\ge \opt(G,\fset)$.
Let $y^*=(y^*_j)_{1\le j\le m}$ be an optimal solution for (LP-Primal) and let $p^*=(p^*(e_i))_{1\le i\le n}$ be an optimal solution for (LP-Dual). From the strong duality, $\sum_{1\le j\le m}v_jy^*_j=\sum_{1\le i\le n}p^*(e_i)=\opt$.
From the complementary slackness, for each $1\le j\le m$, $p^*(Q_j)=\sum_{i: e_i\in Q_j}p^*(e_i)\geq v_j$, and $p^*(Q_j)>v_j$ implies $y^*_j=0$.
We will show that, if we set, for each edge $e_i\in E(G)$, its price as $p^*(i)$, then we will obtain worst-case revenue at least $(2/3)\cdot\opt$, which is at least $(2/3)\cdot\opt(G,\fset)$, with the power of tie-breaking.

We now specify how we will use the power of tie-breaking.
Let $\bset^0$ ($\bset^1,\bset^{1/2}$, resp.) be the set of all buyer $B_j$ with $y_j^*=0$ ($1,\frac{1}{2}$, resp.). 
Note that for each $1\le j\le m$, $p^*(Q_j)\geq v_j$, and for each buyers $B_j$ in $\bset^{1},\bset^{1/2}$, $p^*(Q_j)=v_j$.
First, if some buyer of $\bset^0$ comes, then either $p^*(Q_j)>v_j$, in which case the buyer cannot afford her demand path, or $p^*(Q_j)=v_j$, and in this case we do not let him take her demand path, using the power of tie-breaking. 
Second, if some buyer of $\bset^1$ comes, then $p^*(Q_j)=v_j$, and we let him take her demand path, using the power of tie-breaking.
  
It remains to consider buyers in $\bset^{1/2}$. 
We denote $J=\set{j\mid y^*_j=\frac{1}{2}}$.
From Lemma~\ref{lem:matching-half-integral}, the graph $H$ is the union of vertex-disjoint odd-length cycles.
It is easy to see that the edge set of every cycle can be partitioned into three subsets, such that the edges in each subset are vertex-disjoint. Therefore, the edges of $H$ can be partitioned into three subsets $E(H)=E_1\cup E_2\cup E_3$, such that the edges in set $E_w$ do not share vertices, for each $w\in \set{1,2,3}$.
Note that each edge of $H$ corresponds to a buyer $B_j$ and a demand path $Q_j$. We then define the weight of an edge $e\in E(H)$ as the value of the demand path $Q_j$ that it corresponds to, and we define the weight of $E_w$ as the total weight of all edges of $E_w$, for each $w\in \set{1,2,3}$.
Then the total weight of all edges in $H$ is $\sum_{j\in J}v_j$.
Assume without loss of generality that $E_1$ has the largest weight among $E_1,E_2,E_3$, then the total weight of $E_1$ is at least $\frac 1 3\cdot \sum_{j\in J}v_j$.
Whenever some buyer of $\bset^{1/2}$ that corresponds to an edge of $E_1$ comes, we let him take her demand path, using the power of tie-breaking.
Whenever some buyer of $\bset^{1/2}$ that corresponds to an edge of $E_2,E_3$ comes, we do not let him take her demand path, using the power of tie-breaking.

Clearly, in the above way of using the power of tie breaking, eventually buyers of $\bset^1$ and buyers of $\bset^{1/2}$ that correspond to an edge of $E_1$ will get their demand paths, at price $p^*$.
Therefore, the revenue we obtain is at least
$\sum_{B_j\in \bset^1}v_j+\frac{1}{3}\cdot \sum_{j\in J}v_j\geq \frac{2}{3}\cdot\left(\sum_{B_j\in \bset^1}v_j+\frac{1}{2}\cdot \sum_{j\in J}v_j\right)=\frac{2}{3}\cdot \optwel.$
\end{proof}



We complement Theorem~\ref{thm:star2} with the following theorem. 
\begin{theorem}
	\label{thm: star lower bound}
	For any $\eps>0$, there is a star graph $G$ together with a buyer profile $\fset$, such that any set of prices on edges of $G$ can achieve worst-case revenue at most $(\frac{2}{3}+\eps)\cdot\opt(G,\fset)$, even with the power of tie-breaking.
\end{theorem}
\begin{proof}
	Consider a star graph with four edges $e_1,e_2,e_3,e_4$.
	The buyer-profile $\fset$ is described as follows:
	\begin{itemize}
		\item Buyer $B_1$ demands the path $Q_1$ consisting of edges $e_1, e_2$, with value $v_1=1$;
		\item Buyer $B_2$ demands the path $Q_2$ consisting of edges $e_1, e_3$, with value $v_2=2+\eps'$;
		\item Buyer $B_3$ demands the path $Q_3$ consisting of edges $e_1,e_4$, with value $v_3=2+\eps'$;
		\item Buyer $B_4$ demands the path $Q_4$ consisting of edges $e_3,e_4$, with value $v_4=2$.
	\end{itemize}
	It is clear that the optimal allocation is assigning the edges $e_1,e_2$ to $B_1$, and assigning the edges $e_3,e_4$ to $B_4$, and the optimal welfare is $\optwel(G,\fset)=3$. However, we will show that any set of prices on the edges may achieve the worst-case revenue at most $2+\eps'$, even with the power of tie-breaking. Setting $\eps'=3\eps$, this implies Theorem~\ref{thm: star lower bound}.
	
	Let $\set{p(e_i)}_{1\le i\le 4}$ be any set of prices.
	If $p(Q_1)>1$, then the buyer $B_1$ cannot afford her demand path $Q_1$. Since each pair of paths in $Q_2, Q_3, Q_4$ shares an edge, at most one of buyers $B_2, B_3, B_4$ may get her demand path, so the revenue is at most $2+\eps'$. 
	If $p(Q_4)>2$, then via similar arguments we can show that the revenue is at most $2+\eps'$. 
	Consider now the case where $p(Q_1)\le 1$ and $p(Q_4)\le 2$. We have $p(e_1)\le 1$, and one of $p(e_3),p(e_4)$ is at most $1$. Assume w.l.o.g. that $p(e_3)\le 1$. We let the buyer $B_3$ comes first. 
	Note that $p(Q_3)=p(e_1)+p(e_3)\le 2<2+\eps'$. Therefore, $B_3$ will get her demand path at price at most $2$, and later on no other buyer may get her path. Altogether, the worst-case revenue for any set $\set{p(e_i)}_{1\le i\le 4}$  of prices is at most $2+\eps'$. This completes the proof of Theorem~\ref{thm: star lower bound}.
\end{proof}


We also consider the case where we do not have the power of tie-breaking in the following theorem.
\begin{theorem}
\label{thm:star}
For any $\epsilon>0$, there is an efficient algorithm, that, given any star graph $G$ and any buyer-profile $\fset=\set{(Q_j,v_j)}_{1\le j\le m}$, computes a set of prices on edges of $G$ that achieves the worst-case revenue at least $(\frac{1}{2}-\epsilon)\cdot\opt(G,\fset)$, even without the power of tie-breaking.
\end{theorem}

\begin{proof}
We first show that we can efficiently compute the optimal allocation. \todo{Should be removed?}

Let $\qset$ be the set of paths in the optimal allocation, so $\optwel=\sum_{Q_j\in \qset}v_j$.
We set the prices on the edges of $G$ as follows. 
For each path $Q_j\in \qset$, if it contains a single edge $e_i$, then we set the price of $e_i$ to be $(1-\epsilon)\cdot v_j$; if it contains two edges $e_i,e_{i'}$, then we set the price of both $e_i$ and $e_{i'}$ to be $(\frac{1}{2}-\epsilon)\cdot v_j$.
For each edges that does not belong to any path of $\qset$, we set its price to be $+\infty$.
	
We now show that the above prices will achieve worst-case revenue at least $(\frac{1}{2}-\epsilon)\cdot\optwel(G,\fset)$, even without the power of tie-breaking. For a path $Q_j$ that contains a single edges $e_i$, it is clear that no matter in what order come the buyers, this edge will be taken by some buyer (not necessarily $B_j$) at price $v_j$.
For a path $Q_{j'}$ that contains two edges $e_{i},e_{i'}$, since the price for each of the edges is $(\frac{1}{2}-\epsilon)\cdot v_{j'}$, and the buyer $j'$ demands both of them with value $v_j$, it is clear that no matter in what order come the buyers, at least one of $e_{i},e_{i'}$ will be taken by some buyer (not necessarily $B_{j'}$) at price $(\frac{1}{2}-\epsilon)\cdot v_{j'}$. Altogether, we conclude that the revenue guaranteed by the pricing is at least $(\frac{1}{2}-\epsilon)\cdot\optwel(G,\fset)$.
\end{proof}







\subsubsection{Proof of Lemma~\ref{lem:matching-half-integral}}
\label{sec: proof of matching-half-integral}

In this section we provide the proof of Lemma~\ref{lem:matching-half-integral} for completeness.

Let $y$ be any optimal solution of (LP-Primal) that is an extreme point of the polytope defined by (LP-Primal).
Denote $J=\set{j\mid 0<y_j<1}$. We define a graph $\hat H$ according to $ J$ as follows. 
The vertex set of $\hat H$ contains
(i) a vertex $u_i$ for each edge $e_i\in E(G)$; and
(ii) a vertex $\hat u_i$, for all $1\le i\le n$ such that there exists a buyer $B_j$ with $j\in  J$ whose demand path $Q_j$ contains a single edge $e_i$.
In other words, $V(\hat H)=\set{u_1,\ldots,u_n}\cup \set{\hat u_i\mid \exists j\in  J, Q_j=(e_{i})}$.
The edge set of $\hat H$ contains
(i) an edge $(u_i,u_{i'})$ for each demand path $Q_j=(e_{i},e_{i'})$ with $j\in  J$; and
(ii) an edge $(u_i,\hat u_{i})$ for each demand path $Q_j=(e_{i})$ with $j\in  J$.
In other words, $E(\hat H)=\set{(u_i,u_{i'})\mid \exists j\in  J, Q_j=(e_{i},e_{i'})}\cup \set{(u_i,\hat u_{i})\mid \exists j\in  J, Q_j=(e_{i})}$.

We say that a graph is \emph{Eulerian} iff the degree for each vertex is even. It is folklore that every Eulerian graph contains a trail that visits each edge once.
We use the following claim and its simple corollary.
\begin{claim}
\label{clm: no eulerian subgraph}
$\hat H$ does not contain an Eulerian subgraph with even number of edges.
\end{claim}
\begin{proof}
Assume the contrast that graph $\hat H$ does contain an Eulerian subgraph, and let $(u_{r_1},\ldots, u_{r_t},u_{r_1})$ be the trail that visits each edge of this Eulerian subgraph exactly once (note that such a trail may not contain vertices of $\set{\hat u_i\mid \exists j\in  J, Q_j=(e_{i})}$). 
Define 
$$\hat J_0=\set{j\mid Q_j=(e_i,e_{i'}), \text{ s.t. } \set{r_k,r_{k+1}}=\set{i,i'}\text{ for some even }1\le k\le t};$$ 
and
$$\hat J_1=\set{j\mid Q_j=(e_i,e_{i'}), \text{ s.t. } \exists\text{ odd }k, \set{r_k,r_{k+1}}=\set{i,i'}}.$$
Clearly, sets $\hat J_0$ and  $\hat J_1$ are disjoint.
We define  $z\in \set{-1,0,1}^m$ to be the $m$-dimentional vector, such that, for each $1\le j\le m$, $z_j=1$ iff $j\in \hat J_0$, $z_j=-1$ iff $j\in \hat J_1$, and $z_j=0$ otherwise. 
Let $\eps$ be any constant such that $0<\eps<\min\set{y_j,1-y_j \mid j\in J}$. 
Clearly, vectors $y+\epsilon z$ and $y-\epsilon z$ are both feasible solutions of (LP-Primal). This contradicts the fact that $y$ is an extreme point of the polytope defined by (LP-Primal).
\end{proof}


As a corollary, all cycles of $\hat H$ contains odd number of edges, and all odd-cycles in $\hat H$ are vertex-disjoint. We further prove the following claim.
\begin{claim}
\label{clm: odd cycle in disjoint component}
Every odd cycle of $\hat H$ belongs to a distinct connected component of $\hat H$.
\end{claim}
\begin{proof}
If $\hat H$ does not contain any odd cycle or only contains one odd cycle, then there is nothing to prove. Assume the contrast that $\hat H$ contains two odd-cycles $C,C'$ lying in the same connected component of $\hat H$. Let $P$ be a path connecting a vertex $u$ of $C$ to a vertex $u'$ of $C'$.
Let $V(C)=\set{u,u_{i_1},\ldots,u_{i_r}}$, $V(C')=\set{u',u_{i'_1},\ldots,u_{i'_s}}$, and 
$V(P)=\set{u,u_{i''_1},\ldots,u_{i''_t},u'}$, where $r,s$ are even and the vertices are indexed according to the order in which they appear on $C$, $C'$ or $P$. 
Define 
$$ J_0=\set{j\mid Q_j=(e_i,e_{i'}), \text{ s.t. } \set{i_k,i_{k+1}}=\set{i,i'}\text{ for some even }0\le k\le r};$$ 
$$ J_1=\set{j\mid Q_j=(e_i,e_{i'}), \text{ s.t. } \set{i_k,i_{k+1}}=\set{i,i'}\text{ for some odd }0\le k\le r};$$ 
$$ J_0'=\set{j\mid Q_j=(e_i,e_{i'}), \text{ s.t. } \set{i_k,i_{k+1}}=\set{i,i'}\text{ for some even }0\le k\le s};$$
$$ J_1'=\set{j\mid Q_j=(e_i,e_{i'}), \text{ s.t. } \set{i_k,i_{k+1}}=\set{i,i'}\text{ for some odd }0\le k\le s};$$ 
$$\quad \quad J_0''=\set{j\mid Q_j=(e_i,e_{i'}), \text{ s.t. } \set{i_k,i_{k+1}}=\set{i,i'}\text{ for some even }0\le k\le t}; \text{ and}$$
$$ J_1''=\set{j\mid Q_j=(e_i,e_{i'}), \text{ s.t. } \set{i_k,i_{k+1}}=\set{i,i'}\text{ for some odd }0\le k\le t};$$ 
Let $z\in \set{0,1}^m$ be the vector such that for each $1\le j\le m$, $z_j=1$ iff $j\in  J_0$, $z_j=-1$ iff $j\in  J_1$, and $z_j=0$ otherwise.
We define  vectors $z',z''$ according to sets $ J'_0,  J'_1$ and sets $ J''_0,  J''_1$ similarly.
Let $\eps$ be any constant such that $0<\eps<\min\set{y_j,1-y_j \mid j\in  J}$. 
If $t$ is odd, then we let $\tilde z=\epsilon z+ \epsilon z'-2\epsilon z''$; if $t$ is even, then we let $\tilde z=\epsilon z- \epsilon z'-2\epsilon z''$.
Clearly, vectors $y+\tilde z$ and $y-\tilde z$ are both feasible solutions of (LP-Primal). This contradicts the fact that $y$ is an extreme point of the polytope defined by (LP-Primal).
\end{proof}

As a corollary, each connected component of $\hat H$ is either a tree itself, or the union of an odd cycle with some disjoint trees, each sharing a distinct vertex with the cycle. contains odd number of edges, and all odd-cycles in $\hat H$ are vertex-disjoint. We further prove the following claim.

\begin{claim}
\label{clm: no tree component}
No connected component of $\hat H$ is a tree.
\end{claim}
\begin{proof}
Assume the contrast that $\hat H$ has a connected component that is a tree. Let $T$ be such a tree and we root $T$ at an arbitrary vertex of $T$.
We say that an edge $(u',u'')$ (where $u'$ is the parent vertex of $u''$ in $T$) of $T$ is a \emph{type-$0$} edge iff the tree-distance between $u$ and $u'$ in $T$ is even; otherwise we say that it is a \emph{type-$1$} edge.
We define 
$ J_0=\set{j\mid Q_j=(e_i,e_{i'}), \text{ s.t. } (u_i,u_{i'})\text{ is a type-0 edge}}$, 
and
$ J_1=\set{j\mid Q_j=(e_i,e_{i'}), \text{ s.t. } (u_i,u_{i'})\text{ is a type-1 edge}}$.
Claim~\ref{clm: no tree component} follows from similar arguments in the proof of Claim~\ref{clm: no eulerian subgraph}.
\end{proof}

Via similar arguments in the proof of Claim~\ref{clm: odd cycle in disjoint component}, we can prove the following claim.
\begin{claim}
\label{clm: no odd cycle plus something component}
No connected component of $\hat H$ contains an odd-cycle and at least one non-cycle edge.
\end{claim}

Combining Claim~\ref{clm: no eulerian subgraph}, Claim \ref{clm: odd cycle in disjoint component}, Claim~\ref{clm: no tree component} and Claim~\ref{clm: no odd cycle plus something component}, every connected component of $\hat H$ is a single odd-cycle.
It remains to show that all coordinates of $\set{y_j}_{j\in  J}$ are $1/2$. Consider an odd cycle $C$ with $V(C)=\set{u_{i_1},\ldots,u_{i_r}}$ (where $r$ is odd), where the vertices are indexed in the same order in which they appear on $C$. 
For each $1\le t\le r$, let $Q_{j_t}$ be the path that contains edges $e_{i_t},e_{i_{t+1}}$. 
Via similar arguments in the proof of Claim~\ref{clm: odd cycle in disjoint component}, we can show that $y_{j_t}+y_{j_{t+1}}=1$ for all $1\le t\le r$.  Since $r$ is odd, we conclude that $y_{j_t}=1/2$ for all $1\le t\le r$. This completes the proof of Lemma~\ref{lem:matching-half-integral}.










%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%


\iffalse
We start with any optimal fractional solution $y$ from the LP. Assume that every edge is fully allocated, i.e. $\sum_{j: e_i\in Q_j}y_j=1$ for each edge $e_i$. This is without loss of generality since for every path on the graph we can add a dummy buyer with value $0$, and this will not change the optimal welfare and the prices in the dual LP.


Construct the following dual graph $G'$ of the star graph $G$ according to the fractional allocation $y$. For each edge $e_i\in G$, there is a corresponding vertex $i\in G$. For each path $Q_j=(e_i,e_{i'})$ with allocation $y_j>0$, there is an edge $e'=(i,i')\in G'$ with weight $w(e')=y_j$ and value $v_j$; if the path $Q_j=(e_i)$ contains only a single edge, there is a self loop $e'=(i,i)\in G'$ with weight $w(e')=y_j$. Since each edge is fully allocated in $G$, the sum of weight of the edges connected to any vertex in $G'$ is 1. An example of the transformation is shown in Figure~\ref{fig:startograph}, where orange paths have positive allocation.
\begin{figure}[h]
\centering
\includegraphics[width=0.7\columnwidth]{startograph.pdf}
\znote{subfigure}
\caption{An example of the dual graph of paths on the star.\label{fig:startograph}}
\end{figure}


For any isolated edge $(i,i')\in G'$ that is not connected to any other edge, since the sum of weight of the edges connected to any vertex in $G'$ is 1, the allocation of corresponding path $(e_i,e_{i'})$ is also 1. For any cycle in $G'$ with odd number of edges, if there is no other edge connected to it, the only case where the sum of weight of the edges connected to any vertex in such isolated odd cycle is 1 is when the weight of all edges of the odd cycle is $\frac{1}{2}$, and the allocation of the corresponding path is also $\frac{1}{2}$. To prove that there exists an optimal half-integral solution, we only need to show that there exists an alternative assignment of weights on the edges, such that the sum of weighted value of edges is unchanged, and the graph of edges with positive weight only contains isolated edges and isolated odd cycles.

We start with any optimal weight assignment $w$ on the edges in $G'$. If $G'$ contains any even-length cycle $i_1\to i_2\to\cdots\to i_{2k}\to i_{2k+1}=i_1$ ignoring self-loops, the weight of each edge $(i_{t},i_{t+1})$ must be in range $(0,1)$ since the total weight of the edges connected to any vertex in $G'$ is 1. Define $\e=\min_{1\leq t\leq 2k}\min(w(i_t,i_{t+1}),1-w(i_t,i_{t+1}))$ be the smallest difference between the weight of any edge in the cycle and 0 or 1. Let $w'$ be the following assignment of weights on the edges: for any edge $e'\in G'$ that is not in the cycle, $w'(e')=w(e')$; for any integer $1\leq\ell\leq k$, $w'(i_{2\ell-1},i_{2\ell})=w(i_{2\ell-1},i_{2\ell})+\e$, $w'(i_{2\ell},i_{2\ell+1})=w(i_{2\ell},i_{2\ell+1})-\e$. Let $w''$ be the following weight assignment on the edges: for any edge $e'\in G'$ that is not in the cycle, $w''(e')=w(e')$; for any integer $1\leq\ell\leq k$, $w''(i_{2\ell-1},i_{2\ell})=w(i_{2\ell-1},i_{2\ell})-\e$, $w''(i_{2\ell},i_{2\ell+1})=w(i_{2\ell},i_{2\ell+1})+\e$. Intuitively, in $w'$ and $w''$, for each pair of connected edges in the cycle, the weight of one edge reduces by $\e$, while the weight of the other edge increases by $\e$. See Figure~\ref{fig:evencycle} for a transformation example. 
\begin{figure}[h]
\centering
\includegraphics[width=0.7\columnwidth]{evencycle.pdf}
\caption{An example of the two possible perturbations of an even cycle.\label{fig:evencycle}}
\end{figure}



Then by the definition of $\e$, the weight of each edge in $w'$ and $w''$ is still between 0 and 1, while the total weight of the edges connected to any vertex is still 1. Thus $w'$ and $w''$ are two feasible weight assignments on edges, and the average of $w'(e')$ and $w''(e')$ on any edge $e'\in G'$ is exactly $w(e')$. Therefore one of $w'$ and $w''$ has at least the same total weighted value as $w$; actually since $w$ is optimal, both $w'$ and $w''$ has the same total weighted value as $w$. Notice that by definition of $\e$, there exists an edge $(i_t,i_{t+1})$ such that its weight in one of $w'$ and $w''$ (without loss of generality assume it's $w'$) is either 0 or 1. If $w'(i_t,i_{t+1})=0$, then the number of edges of positive weight in $w'$ is smaller than $w$; if $w'(i_t,i_{t+1})=1$, then since the total weight of the edges connected to $i_t$ is still 1, we know that $w'(i_{i-1},i_t)=0$, thus the number of edges of positive weight in $w'$ is smaller than $w$. This means that we can then replace the optimal allocation $w$ with $w'$, and after repeating the operation for finite number of rounds 
the remaining graph $G'$ will have no even cycle.



What's the structure of the graph $G'$ with no even cycle? Each connected component must be a ``tree of odd cycles'', which can be constructed by starting with a tree $T$, and replace some nodes of the tree by cycles of odd length. Notice that since each edge in $G'$ has a positive weight, each leaf node in $T$ must be replaced by a self-loop in $G'$, otherwise such connected component must be an isolated edge. If $G'$ does not only contain isolated edges and isolated cycles, then $G'$ must contain a subgraph $H$ with the following structure: $H$ consists of two odd cycles $C_1:i_1\to i_2\to\cdots\to i_{2k+1}\to i_{2k+2}=i_1)$ and $C_2:i'_1\to i'_2\to \cdots\to i'_{2\ell+1}\to i'_{2\ell+2}=i'_1$, while there is a stem path $L:i_1=i''_1\to i''_2\to\cdots\to i''_s=i'_1$ between the two cycles. We allow the length of the stem path to be zero. If a cycle is a self loop, we will merge it with the stem path: for example, if $C_2$ is a self loop, we will set $L$ to be $i_1=i''_1\to i''_2\to\cdots\to i''_s\to i''_s$. In the later proof, when we refer to a cycle $C_i$, we will assume that it has length at least 3. Define $\e=\min\left(\frac{1}{2}\min_{e'\in  L}\min(w(e'),1-w(e')),\min_{e'\in H\setminus L}\min(w(e'),1-w(e'))\right)$ be the smallest difference between the weight of any edge in the subgraph and 0 or 1, while the difference doubled for the edges not on the stem. Similar to the case of even cycle, we find two different weight allocations of edges $w'$ and $w''$, such that 
\begin{itemize}
    \item The weight of each edge not in $H$ is unchanged in $w'$ and $w''$ compared to $w$;
    \item The weight of each edge in $L$ increases or decreases by $2\e$ in $w'$ and $w''$;
    \item The weight of each edge in $H\setminus L$ increases or decreases by $\e$ in $w'$ and $w''$;
    \item The total weight of the edges connected to any vertex is still 1 in $w'$ and $w''$.
 \end{itemize}
See Figure~\ref{fig:oddcycle} for a transformation example without self-loop, and Figure~\ref{fig:oddselfcycle} for a transformation example with one of the odd cycles being a self-loop. 
\begin{figure}[h]
\centering
\includegraphics[width=0.7\columnwidth]{oddcycle.pdf}
\caption{An example of the two possible perturbations of two connected odd cycles without self-loop.\label{fig:oddcycle}}
\end{figure}
\begin{figure}[h]
\centering
\includegraphics[width=0.7\columnwidth]{oddselfcycle.pdf}
\caption{An example of the two possible perturbations of two connected odd cycles with self-loop.\label{fig:oddselfcycle}}
\end{figure}
The same as in the even-cycle case, the weight of each edge in $w'$ and $w''$ is still between 0 and 1. Thus $w'$ and $w''$ are two feasible weight assignments on edges, and the average of $w'(e')$ and $w''(e')$ on any edge $e'\in G'$ is exactly $w(e')$, then both $w'$ and $w''$ has the same total weighted value as $w$. Notice that by definition of $\e$, there exists an edge in $H$ such that its weight in one of $w'$ and $w''$ (without loss of generality assume it's $w'$) is either 0 or 1. Using the same argument as in the even-cycle case the number of edges of positive weight in $w'$ is smaller than $w$. Then we can then replace the optimal allocation $w$ with $w'$, and after repeating the operation for finite number of rounds the remaining graph $G'$ will have no subgraph with such a structure like $H$.

After the above operations, we finally get a graph $G'$ such that each of its connected component is either an edge or an odd cycle. This finishes the proof of the lemma.

\fi

%\ytnote{TODO: add spider case by proving a reduction to the star case.}


==> star_and_spider_new.tex <==
\subsection{Stars and Spiders}\label{sec:star_and_spider}
We first consider the case where the underlying graph $G$ is a star or a spider graph. A \emph{spider} $G$ is a tree with one vertex $u$ of degree at least 3 and all others with degree at most 2. In other words, $E(G)$ can be decomposed into $k$ paths, where any two paths only intersect at $u$. Star is a special spider graph, where all vertices other than $u$ has degree 1.
See \Cref{fig:star_spider} for an example.

\begin{figure}[h]
	\centering
	\subfigure[A star.]{\scalebox{0.08}{\includegraphics{star.jpg}}}
	\hspace{5pt}
	\subfigure[A spider.]{\scalebox{0.08}{\includegraphics{spider.jpg}}}
	\caption{An illustration of stars and spiders.\label{fig:star_spider}}
\end{figure}

As a warm-up, we first prove that the competitive ratio of any star graph is at most $3/2$. For star graphs, let $E(G)=\{e_1,\ldots,e_m\}$.

\begin{theorem}
\label{thm:star2}
$\ratio(\starr)\leq 3/2$. Moreover, the set of prices that achieves the competitive ratio $3/2$ can be computed efficiently.
\end{theorem}

Here is our plan for the proof: We round the optimal solution of (LP-Primal) to get a feasible integral solution with a total value of at least $2/3\cdot \opt$, and then apply Lemma~\ref{lem:rounding}. One crucial lemma we use here is that, if the input graph is a star, then (LP-Primal) contains a half-integral optimal solution, i.e. an vector in $\{0,\frac{1}{2},1\}^n$ that achieves the optimal objective value. This lemma was also proved in~\cite{matchingLP}. 
For completeness, we include a proof of Lemma~\ref{lem:matching-half-integral} in Appendix~\ref{subsec:appx_star_and_spider}. 

\begin{lemma}\label{lem:matching-half-integral}\cite{matchingLP}
If $G$ is a star graph, then (LP-Primal) is half-integral, and for each optimal solution $y^*\in \set{0,\frac 1 2,1}^{n}$, if we denote $J^*=\set{j\mid y^*_j=\frac{1}{2}}$ and define the graph $H$ as $V(H)=\set{u_i\mid e_i\in \bigcup_{j\in J^*}Q_j}$ and $E(H)=\set{(u_i,u_{i'})\mid \exists j\in J^*, Q_j=\{e_i,e_{i'}\}}$, then $H$ is the union of vertex-disjoint odd-length cycles.
\end{lemma}

\begin{prevproof}{Theorem}{thm:star2}
Without loss of generality, we assume that for every $i,i'\in [m]$, at most one buyer has demand path $\{e_i,e_{i'}\}$, otherwise we only keep the buyer with the largest value. Let $y^*$ be the optimal solution of (LP-Primal). Let $\bset^0$ ($\bset^1,\bset^{1/2}$, resp.) be the set of all buyer $j$ with $y_j^*=0$ ($1,\frac{1}{2}$, resp.).
For buyers in $\bset^{1/2}$, define the graph $H$ as $V(H)=\set{u_i\mid e_i\in \bigcup_{j\in \bset^{1/2}}Q_j}$ and $E(H)=\set{(u_i,u_{i'})\mid \exists j\in \bset^{1/2}, Q_j=\{e_i,e_{i'}\}}$, then from Lemma~\ref{lem:matching-half-integral}, $H$ is the union of vertex-disjoint odd-length cycles. It's easy to verify that the edge set of every cycle can be partitioned into three subsets, such that the edges in each subset are vertex-disjoint. Therefore, the edges of $H$ can be partitioned into three subsets $E(H)=E_1\cup E_2\cup E_3$, such that the edges in set $E_w$ do not share vertices, for each $w\in \set{1,2,3}$.
Note that each edge of $H$ corresponds to the demand path $Q_j$ of a unique buyer $j\in \bset^{1/2}$. For simplicity we denote $\hat{e}_j$ the edge of $H$ matched to buyer $j$. Without loss of generality, assume $\sum_{j:\hat{e}_j\in E_1}\geq \frac{1}{3}\cdot \sum_{j\in \bset^{1/2}}v_j$. We construct a feasible integral solution $y$ as follows. For every $j\in \bset^1$, let $y_j=y_j^*=1$; For every $j\in \bset^{1/2}$ such that $\hat{e}_j\in E_1$, let $y_j=1$; For other $j$, let $y_j=0$. Note that the fact that edges in $E_1$ is node-disjoint implies that demand paths $\{Q_j\mid \hat{e}_j\in E_1\}$ are edge-disjoint. Also, since $y^*$ is feasible, it's clear that the demand path for buyer $j\in \bset^1$ does not intersect with the demand path for $j\in \bset^{1/2}$. Thus $y$ is feasible.

To finish the proof, we notice that
$$\sum_{j:y_j=1}v_j\geq \sum_{j\in \bset^1}v_j+\frac{1}{3}\cdot \sum_{j\in \bset^{1/2}}v_j\geq \frac{2}{3}\cdot\left(\sum_{B_j\in \bset^1}v_j+\frac{1}{2}\cdot \sum_{j\in \bset^{1/2}}v_j\right)=\frac{2}{3}\cdot \optlp\geq \frac{2}{3}\optwel.$$
Applying Lemma~\ref{lem:rounding} finishes the proof.
\end{prevproof}

We prove in the following theorem that the $3/2$ competitive ratio is tight for star graphs. 
\begin{theorem}
	\label{thm: star lower bound}
	For any $\eps>0$, $\ratio(\starr)>3/2-\eps$.
\end{theorem}
\begin{proof}
	Consider a star graph with four edges $e_1,e_2,e_3,e_4$.
	The instance $\fset$ is described as follows:
	\begin{itemize}
		\item Buyer 1 demands the path $Q_1$ consisting of edges $e_1, e_2$, with value $v_1=1$;
		\item Buyer 2 demands the path $Q_2$ consisting of edges $e_1, e_3$, with value $v_2=2+\eps$;
		\item Buyer 3 demands the path $Q_3$ consisting of edges $e_1,e_4$, with value $v_3=2+\eps$;
		\item Buyer 4 demands the path $Q_4$ consisting of edges $e_3,e_4$, with value $v_4=2$.
	\end{itemize}
	It is clear that the optimal allocation is assigning the edges $e_1,e_2$ to buyer 1, and assigning the edges $e_3,e_4$ to buyer 4. The optimal welfare is $\optwel(G,\fset)=3$. However, we will show that any set of prices on the edges achieve the worst-case welfare at most $2+\eps$. Then $\ratio(\text{Star})\geq \frac{3}{2+\eps}>\frac{3}{2}-\eps$.
	
	Let $\set{p_i}_{1\le i\le 4}$ be any set of prices.
	If $p(Q_1)>1$, then buyer 1 cannot afford her demand path $Q_1$. Since each pair of paths in $Q_2, Q_3, Q_4$ shares an edge, at most one of buyers $2,3,4$ may get her demand path, so the welfare is at most $2+\eps$. 
	If $p(Q_4)>2$, then via similar arguments we can show that the welfare is at most $2+\eps$. 
	Consider now the case where $p(Q_1)=p_1+p_2\le 1$ and $p(Q_4)=p_3+p_4\le 2$. We have $p_1\le 1$, and one of $p_3,p_4$ is at most $1$. Assume w.l.o.g. that $p_3\le 1$. We let buyer 3 comes first. 
	Note that $p(Q_3)=p_1+p_3\le 2<2+\eps$. Therefore, buyer 3 will get her demand path, and later on no other buyer may get her path. Altogether, the worst-case welfare for any set of prices is at most $2+\eps$. This completes the proof of Theorem~\ref{thm: star lower bound}.
\end{proof}

Now we come to spider graphs. We prove that the competitive ratio is at most $3/2$ for any spider graph. Note that the ratio is tight according to Theorem~\ref{thm: star lower bound}.

\begin{theorem}
\label{thm:spiderimproved}
$\ratio(\spider)\leq 3/2$. Moreover, the set of prices that achieves the competitive ratio $3/2$ can be computed efficiently.
\end{theorem}

Similar to the proof of Theorem~\ref{thm:star2}, we prove in the following lemma that (LP-Primal) has a half-integral optimal solution. The proof uses Lemma~\ref{lem:matching-half-integral}
and is postponed to Appendix~\ref{subsec:appx_star_and_spider}.

\begin{lemma}\label{lem:spider-half-integral} 
If $G$ is a spider graph, then (LP-Primal) has a half-integral optimal solution. Moreover, such a solution can be computed efficiently.
\end{lemma}

\begin{prevproof}{Theorem}{thm:spiderimproved}
Let $y^*$ be a half-integral optimal solution of (LP-Primal) given by Lemma~\ref{lem:spider-half-integral}. Denote $\bset^{1/2}=\set{j\mid y^*_j=1/2}$ and $\bset^1=\set{j\mid y^*_j=1}$. Since $y^*$ is feasible, paths $\set{Q_j\mid j\in \bset^1}$ are edge-disjoint, and they do not share the same edge with paths $\set{Q_j\mid j\in \bset^{1/2}}$. We will show that we can efficiently compute a subset $\bset'\subseteq \bset^{1/2}$, such that (i) the paths $\set{Q_j\mid j\in \bset'}$ are edge-disjoint; and (ii) the total value of paths in $\set{Q_j\mid j\in \bset'}$ is at least $\frac{1}{3}\cdot \sum_{j\in \bset^{1/2}}v_j$. If so, we let $y_j=\ind[j\in \bset^1\cup \bset']$. Then $y=\{y_j\}_{j\in [n]}$ is a feasible integral solution of (LP-Primal). Moreover,
$$\sum_{j:y_j=1}v_j\geq \sum_{j\in \bset^1}v_j+\frac{1}{3}\cdot \sum_{j\in \bset^{1/2}}v_j\geq \frac{2}{3}\cdot\left(\sum_{B_j\in \bset^1}v_j+\frac{1}{2}\cdot \sum_{j\in \bset^{1/2}}v_j\right)=\frac{2}{3}\cdot \optlp\geq \frac{2}{3}\optwel.$$
Thus applying Lemma~\ref{lem:rounding} finishes the proof.

To find a subset $\bset'$ that satisfies both properties, we prove the following structural lemma for trees. The proof of the lemma is postponed to Appendix~\ref{subsec:appx_star_and_spider}.

\begin{lemma}\label{lem:tree-coloring}
Let $T$ be a tree, let $d\geq 2$ be an integer and let $\qset$ be a set of paths in $T$, such that every edge of $T$ appears in at most $d$ paths of $\qset$, then we can efficiently compute a partition of $\qset$ into $d+1$ subsets $\qset_1,\ldots,\qset_{d+1}$, such that for every $1\le i\le d+1$, paths in $\qset_i$ are edge-disjoint.
\end{lemma}

Now since $y^*$ is a feasible solution of (LP-Primal), $y^*_j=1/2$ for each $j\in \bset^{1/2}$. Thus every edge of $G$ is contained in at most $2$ paths in $\qset=\{Q_j\mid j\in \bset^{1/2}\}$. By Lemma~\ref{lem:spider-half-integral}, we can efficiently obtain a partition $(\qset_1,\qset_2, \qset_3)$ of $\qset$, such that for each $1\le i\le 3$, paths in $\qset_i$ are edge-disjoint.
Therefore, at least one of sets $\qset_1,\qset_2,\qset_3$ contains edge-disjoint paths of total value at least $\frac{1}{3}\sum_{j\in \bset^{1/2}}v_j$. This completes the proof of Theorem~\ref{thm:spiderimproved}.
\end{prevproof}






==> tree.tex <==


\subsection{Trees}\label{sec:tree}

Now we consider trees. In this section we prove that the competitive ratio of any tree graph is at most 3.

\begin{theorem}
\label{thm: tree}
$\ratio(\tree)\leq 3$. Moreover, the prices that achieve the competitive ratio 3 can be computed efficiently.
\end{theorem}

The remainder of this section is dedicated to the proof of \Cref{thm: tree}. In Section~\ref{sec:star_and_spider}, we prove that when $G$ is a spider (and star), there exists a half-integral optimal solution for (LP-Primal). This is necessary to achieve a feasible allocation through rounding, whose total welfare is at least $2/3\cdot \opt$. However, this does not hold for general tree graphs. In fact, we show in Lemma~\ref{lem:tree-example} that, for trees, the optimal solution for (LP-Primal) may contain a positive value with an arbitrarily large denominator.

\begin{lemma}\label{lem:tree-example}
For any integer $d>0$, there exists a tree $G$ and an instance $\fset$, such that every coordinate of the unique optimal solution of (LP-Primal) is either $1/d$ or $(d-1)/d$.
\end{lemma}
\begin{proof}
We construct a tree $G$ as follows. The vertex set is $V(G)=\set{u_i,v_i\mid 0\le i\le 2d}$. The edge set is $E(G)=\set{u_0,v_0}\cup \set{(u_i,u_0),(v_i,v_0)\mid 1\le i\le 2d}$.
Consider the following instance $\fset$: It contains (i) for each $1\le j\le 2d$, a buyer $B_j$ that demands the path  $Q_j=(u_j,u_0,v_0,v_j)$ with value $3$; (ii) for each $1\le k\le d$, a buyer $B^u_k$ that demands the path $Q^u_k=(u_{2k-1},u_0,u_{2k})$ with value $2$; and (iii) for each $1\le k\le d$, a buyer $B^v_k$ that demands the path $Q^v_k=(v_{2k},v_0,v_{2k+1})$ with value $2$. See Figure~\ref{fig:d-integral} for an illustration.
It is not hard to see that $G$ is a tree, and in the unique optimal solution $y$ of (LP-Primal), for each path $Q_j$, $y_j=1/d$; and for each path $Q^u_k$ and each path $Q^v_{k'}$, $y_{u,k}=y_{v,k'}=(d-1)/d$.
\begin{figure}[h]
	\centering
	\includegraphics[width=0.4\columnwidth]{d-integral.jpg}
	\caption{An illustration of graph $G$, where paths of $\set{Q_1,\ldots,Q_{2d}}$ are shown in orange, and paths of $\set{Q^u_1,\ldots,Q^u_{k}}\cup \set{Q^v_1,\ldots,Q^v_{k}}$ are shown in purple.\label{fig:d-integral}}
\end{figure}
\end{proof}

To prove Theorem~\ref{thm: tree}, we use a different approach from Section~\ref{sec:star_and_spider}. We prove the following structural lemma, which partitions a set of edge-disjoint paths into two sets, such that each set of paths forms a union of vertex-disjoint spider graphs. And then we apply Theorem~\ref{thm:spiderimproved} to get the desired set of prices. 

\begin{lemma}\label{lem:treetospider}
Let $P_1,\ldots,P_n$ be edge-disjoint paths, such that the graph $G=\bigcup_{j\in [n]}P_j$ is a tree, then the set $\pset=\set{P_1,\ldots,P_n}$ can be partitioned into two sets $\pset=\pset'\cup\pset''$, such that both the graph induced by paths in $\pset'$ and the graph induced by paths in $\pset''$ are the union of vertex-disjoint spiders.
\end{lemma}

\begin{proof}
We choose arbitrarily a vertex $r\in V(G)$ as designate it as the root of the tree.
We iteratively construct a sequence of subsets of  $\pset$ as follows.
We first let $\pset_1$ contains all paths of $\pset$ that contains the vertex $r$.
Then for each $i>1$, as long as $\pset\ne \bigcup_{1\le t\le i-1}\pset_t$, we let $\pset_i$ contains all paths in $\pset\setminus \left(\bigcup_{1\le t\le i-1}\pset_t\right)$ that shares a vertex with a path in $\pset_{i-1}$.
We continue this process until all paths of $\pset$ are included in sets $\pset_1,\ldots,\pset_k$ for some $k$.
See Figure~\ref{fig:spider_decomp} for an illustration.
We then let $\pset'=\bigcup_{0\le t\le \lfloor{k/2}\rfloor}\pset_{2t+1}$ and $\pset''=\bigcup_{1\le t\le \lfloor{k/2}\rfloor}\pset_{2t}$. This completes the construction of the sets $\pset',\pset''$. Clearly, sets $\pset'$ and $\pset''$ partition $\pset$.

\begin{figure}[ht]
\centering
\subfigure[The graph $G$. Paths are shown in distinct colors.]{\scalebox{0.25}{\includegraphics{spider_decomp_layout.jpg}}\label{fig:non_crossing_representation}}
\hspace{1pt}
\subfigure[The paths in $\pset_1$ are shown in dash lines.]{\scalebox{0.25}{\includegraphics{spider_decomp_1.jpg}}}
\subfigure[The paths in $\pset_2$ are shown in dash lines.]{\scalebox{0.25}{\includegraphics{spider_decomp_2.jpg}}}
\hspace{1pt}
\subfigure[The paths in $\pset_3$ are shown in dash lines.]{\scalebox{0.25}{\includegraphics{spider_decomp_3.jpg}}}
\caption{An illustration of decomposing paths into subsets $\pset_1,\pset_2,\pset_3$.\label{fig:spider_decomp}}
\end{figure}

It remains to show that the graph induced by the paths in $\pset'$ is the union of vertex-disjoint spiders. The proof for $\pset''$ is similar.
First, for $0\le t<t'\le \lfloor{k/2}\rfloor$, we show that the paths in $\pset_{2t+1}$ are vertex-disjoint from the paths in $\pset_{2t'+1}$. Assume for contradiction that this is false, and let $P\in \pset_{2t+1}, P'\in \pset_{2t'+1}$ be a pair of paths that share a common vertex. However, according to the process of constructing the sets $\pset_1,\ldots,\pset_k$, if $P$ is included in $\pset_{2t+1}$ while $P'$ is not included in any set of $\pset_1,\ldots,\pset_{2t+1}$, since $P'$ shares a vertex with $P'$, $P'$ should be included in the set $\pset_{2t+2}$ rather than $\pset_{2t'+1}$, a contradiction.
We then show that, for each $0\le t\le \lfloor{k/2}\rfloor$, the paths in $\pset_{2t+1}$ form disjoint spiders. Clearly the paths in $\pset_1$ form a spider, since they are edge-disjoint paths that share only the root $r$ of tree $G$. Consider now some $t\ge 1$.
Let $v,v'$ be any two distinct vertices of $V(\pset_{2t})\cap V(\pset_{2t+1})$. We denote by $\pset_{2t+1}(v)$ ($\pset_{2t+1}(v')$, resp.) the subset of paths in $\pset_{2t+1}$ that contains the vertex $v$ ($v'$, resp.).
We claim that the paths in $\pset_{2t+1}(v)$ are vertex-disjoint from the paths in $\pset_{2t+1}(v')$.
Note that, if the claim is true, since the paths in $\pset_{2t+1}(v)$ only shares a single node $v$ (as otherwise there is a cycle caused by some pair of paths in $\pset_{2t+1}(v)$, a contradiction to the fact that graph $G=\bigcup_{j\in [n]}P_i$ is a tree), it follows that the paths in $\pset_{2t+1}(v)$ form a spider, and altogether, the paths in $\pset'$ form vertex-disjoint spiders.

It remains to prove the claim.
Assume that this is false. Let $P_{2t+1}\in \pset_{2t+1}(v), P'_{2t+1}\in \pset_{2t+1}(v')$ be a pair of paths that shares a common vertex $u$, with $u\ne v,v'$. Note that, from our process of constructing the sets $\pset_1,\ldots,\pset_k$, there are two sequences of paths $P_1,P_2,\ldots,P_{2t}$ and $P'_1,P'_2,\ldots,P'_{2t}$, such that
(i) for each $1\le s\le 2t$, $P_{s}, P'_{s}\in \pset_s$;
(ii) for each $1\le s\le 2t$, $P_{s}$ shares a vertex with $P_{s+1}$, and $P'_{s}$ shares a vertex with $P'_{s+1}$.
Since $P_1$ and $P'_1$ shares the root $r$ of tree $G$, it follows that the graph consisting of paths in $\set{P_s,P'_s \mid 1\le s\le 2t+1}$ contains a cycle, a contradiction to the fact that $G$ is a tree.
\end{proof}

\begin{prevproof}{Theorem}{thm: tree}
Let $\qset^*$ be the subset of $\set{Q_1,\ldots,Q_n}$ that, over all subsets of edge-disjoint paths in $\set{Q_1,\ldots,Q_n}$, maximizes its total value, namely $\opt(G,\fset)=\sum_{Q_j\in \qset^*}v_j$. Clearly, graph $G^*=\bigcup_{Q\in \qset^*}Q$ is the union of a number of disjoint trees. We further partition $\qset^*=\bigcup_{1\le t\le k}\qset^*_t$, such that the union of paths in each $\qset^*_t$ forms a connected component of $G^*$, and is therefore a tree (a subtree of $G$). We then apply Lemma~\ref{lem:treetospider} to each set $\qset^*_t$. Assume the partition for $\qset^*_t$ is $\qset^{(1)}_t\cup \qset^{(2)}_t$ such that $\sum_{Q_j\in \qset^{(1)}_t}v_j\geq \sum_{Q_j\in\qset^{(2)}_t}v_j$. Denote $\hat\qset^*=\bigcup_{1\le t\le k}\qset^{(1)}_t$. Then clearly $\hat G^*=\bigcup_{Q\in \hat\qset^*}Q$ is the union of disjoint spiders and $\sum_{Q_j\in \hat\qset^*}v_j\geq \frac{1}{2}\opt(G,\fset)$. Thus by \Cref{thm:spiderimproved}, there exists a set of prices $p$ that achieves worst-case welfare at least $\frac{1}{3}\opt(G,\fset)$.

It remains to show that such a price vector $p$ can be computed efficiently. Firstly, computing the hindsight optimal solution $\qset^*$ is equivalent to computing the maximum weight edge-disjoint paths in a tree, for which a polynomial-time algorithm exists~\cite{tarjan1985decomposition}. According to the proof of Lemma~\ref{lem:treetospider}, partitioning $\qset^*$ clearly takes polynomial time. Thus the price vector can be computed efficiently by Theorem~\ref{thm:spiderimproved} that the corresponding set of prices can be computed efficiently in spider graphs.
\end{prevproof}



\iffalse
\mingfeinote{move to the no tie-breaking section}
The same reduction works when the seller does not have tie-breaking power. The following theorem follows from \Cref{thm:spider-no-tiebreak}.

\begin{theorem}\label{thm:tree-no-tiebreak}
For any constant $\eps>0$, there is an efficient algorithm, that, given any tree $G$ and any buyer-profile $\fset=\set{(Q_j,v_j)}_{j\in [n]}$, computes a set of prices on edges of $G$ that achieves the worst-case revenue equal at least $(\frac{1}{7}-\eps)\cdot\opt(G,\fset)$, without the power of tie-breaking.
\end{theorem}

\fi



